Distributionally Robust Data Join

Suppose we are given two datasets: a labeled dataset and unlabeled dataset which also has additional auxiliary features not present in the first dataset. What is the most principled way to use these datasets together to construct a predictor? The answer should depend upon whether these datasets are generated by the same or different distributions over their mutual feature sets, and how similar the test distribution will be to either of those distributions. In many applications, the two datasets will likely follow different distributions, but both may be close to the test distribution. We introduce the problem of building a predictor which minimizes the maximum loss over all probability distributions over the original features, auxiliary features, and binary labels, whose Wasserstein distance is $r_1$ away from the empirical distribution over the labeled dataset and $r_2$ away from that of the unlabeled dataset. This can be thought of as a generalization of distributionally robust optimization (DRO), which allows for two data sources, one of which is unlabeled and may contain auxiliary features.

==> k-anchor.tex <==

\section{$k$-anchors}
\subsection{Additional Preliminaries}
Suppose we have $k$ datasets $S_l = \{(x^l_i, a^l_i)\}_{i=1}^{n_l}$ for $l \in [k]$ that each has its own unique set of features $\cA_l$ and one full dataset $S_T = \{(x^T_i, \{a^{T, l}_i\}_{l=1}^{k})\}_{i=1}^{n_T}$ that consists of all the features. For each $l \in [k]$, the corresponding metric is defined as 
\[
    d_l((x,a^l), (x',{a'}^l)) = ||x-x'||_{p} + \kappa_l ||a^l-{a'}^l||_{p_l}.
\]

\[
    d_T((x,\{a^{l}\}_{l}), (x', \{{a'}^l\}_l))) = ||x-x'||_{p} + \sum_{l \in [k]} \kappa_{T,l}  ||a^l-{a'}^l||_{p_l}
\]

And the goal is to find a joint distribution such that it is with in the Wasserstein ball centered at $\tP_{S_l}$ of radiu $r_l$ for each $l \in [k]$ and Wasserstein ball centered at $\tP_{S_T}$ of radius $r_T$. 

In other words,
\begin{align*}
    W(\{S_l\}_{l=1}^k, \{r_l\}_{l=1}^k, S_T, r_T) = \left\{\cQ \in \bP_{\cX, \{\cA_l\}_{l=1}^{n_l}}: \cQ_{\cX, \cA_l} \in B_{d_l}(\tP_{S_l}, r_l) \forall l \in [k], \cQ \in B(S_T, r_T)\right\}
\end{align*}
\subsection{Problem and Duality}
For simplicity, we write $\overline{i} = (i_1, \dots, i_k, i_T)$.
\begin{align}
\begin{split}
     \sup_{\pi}  &\sum_{i_1=1}^{n_1} \dots \sum_{i_k=1}^{n_k} \sum_{i_T=1}^{n_T} \int_{\cX, \cA_1, \dots, \cA_k} \ell(\theta, (x, \{a_{l}\}_{l \in [k]})) \pi_{\overline{i}}(dx, \{da^{l}\}_{l \in [k]}) \\
     \text{s.t.} \quad& \sum_{i_1=1}^{n_1} \dots \sum_{i_k=1}^{n_k} \sum_{i_T=1}^{n_T} \int_{\cX, \cA_1, \dots, \cA_k} d_l(x,a^l, x^l_{i_l}, a^l_{i_l}) \pi_{\overline{i}}(dx, \{da^{l}\}_{l \in [k]}) \le r_l \quad\forall l \in [k]\\
     &\sum_{i_1=1}^{n_1} \dots \sum_{i_k=1}^{n_k} \sum_{i_T=1}^{n_T} \int_{\cX, \cA_1, \dots, \cA_k} d_T((x, \{a^{l}\}_{l \in [k]}), (x^T_{i_T}, \{a^{T,l}_{i_T}\}_{i_T=1}^{n_T})) \pi_{\overline{i}}(dx, \{da^{l}\}_{l \in [k]}) \le r_T \\
    \quad& \sum_{i_1=1}^{n_1} \sum_{i_{l'-1}=1}^{n_{l'-1}}\dots \sum_{i_{l'+1}=1}^{n_{l'+1}} \sum_{i_k=1}^{n_k} \sum_{i_T=1}^{n_T} \int_{\cX, \cA_1, \dots, \cA_k} \pi_{\overline{i}}(dx, \{da^{l}\}_{l \in [k]}) =\frac{1}{n_l} \quad\forall l' \in [k] 
\end{split}
\end{align}
\cj{TODO: fix the coupling constraint}
And the corresponding dual problem is then 
\begin{align}
\begin{split}
    &\inf_{\alpha, \beta} \quad \sum_{l=1}^k \alpha_l r_l + \alpha_T r_T + \frac{1}{n_1}\sum_{i_1=1}^{n_1} \beta^1_i  + \dots + \frac{1}{n_k}\sum_{i_k=1}^{n_k} \beta^k_{i_k} \quad\text{such that} \\
    &\sup_{(x, \{a_{l}\}_{l \in [k]})} \left(\ell(\theta, (x, \{a^{l}\}_{l \in [k]})) - \sum_{l'\in[k]}\alpha_{l'} d^{i_l}_l(x,a^l) - \alpha_T d^{i_T}_{T}(x, \{a^l\}_{l=1}^{n_l})\right) - \sum_{l' \in [k]}\beta^l_{i_l} \le 0 \quad i_1 \in [n_1], \dots, i_k \in [n_k]
\end{split}
\end{align}

As before, we will try to replace the $\sup$. For notational simplicity, we write $\theta[\cX]$ to denote the coordinates that correspond to $\cX$ and likewise for $\theta[\cA_l]$ given a vector $\theta$ whose number of coordinates is the sum of the coordinates in $\cX$ and the number of coordinates in $\cA_l$ for each $l\in [k]$.
\begin{lemma} $\sup_{(x, \{a_{l}\}_{l \in [k]})} \left(\ell(\theta, (x, \{a_{l}\}_{l \in [k]})) - \sum_{l'\in[k]}\alpha_{l'} d^{i_l}_l(x,a_l) - \alpha_T d^{i_T}_{T}(x, \{a_l\}_{l=1}^{n_l})\right)$ evaluates in the following manner. If $||\theta[\cX]||_{p,*} > \sum_{l \in [k]} \alpha_l + \alpha_T$ and $||\theta[\cA_l]||_{p_l,*} > \kappa_l \alpha_l + \kappa_{T,l} \alpha_T$ for each $l \in [k]$, then the expression evaluates to $\infty$. Otherwise, it evaluates to
\[
    \sup_{b \in [0,1]} \inf_{\substack{||q_l||_{*} \le \alpha_l, ||q'_l||_{*} \le \kappa_l \alpha_l \\||q_T||_{*}\le\alpha_T, ||q'_{T,l}||_{*}\le \kappa_{T,l} \alpha_T}} -f^*(b) + (g_1 \square \dots \square g_k \square g_T)(b\theta[\cX]) + \sum_{l \in [k]} (g'_1 \square g'_{T,l})(b\theta[\cA_l])
\]
where 
\[
    g_1(q) = \begin{cases}\langle -x^l, q \rangle \quad\text{if $||q||_{p,*} \le \alpha_l$}\\
    \infty \quad\text{otherwise}
    \end{cases}
\]
\[
    g_T(q) = \begin{cases}\langle -x^T, q \rangle \quad\text{if $||q||_{p,*} \le \alpha_T$}\\
    \infty \quad\text{otherwise} \end{cases}
\]
\[
    g'_l(q) = \begin{cases}\langle -a^l, q \rangle \quad\text{if $||q||_{p_l,*} \le \kappa_l\alpha_l$}\\
    \infty \quad\text{otherwise}
    \end{cases}
\]
\[
    g'_{T,l}(q) = \begin{cases}\langle -a^{T,l}, q \rangle \quad\text{if $||q||_{p_l,*} \le \kappa_{T,l}\alpha_{T}$}\\
    \infty \quad\text{otherwise} \end{cases}
\]
\end{lemma}
\begin{proof}
    Noting that $h$ is convex and thus $h$ is equal to its biconjugate $h^{**}$, we have
\begin{align*}
    &\sup_{(x, \{a_{l}\}_{l \in [k]})} \left(\ell(\theta, (x, \{a_{l}\}_{l \in [k]})) - \sum_{l'\in[k]}\alpha_{l'} d^{i_l}_l(x,a_l) - \alpha_T d^{i_T}_{T}(x, \{a_l\}_{l=1}^{n_l})\right)\\
    &\sup_{(x, \{a_{l}\}_{l \in [k]})} \sup_{b \in [0,1]} \left(\langle b\theta, (x, \{a_{l}\}_{l \in [k]}) \rangle -f^*(b) -  \sum_{l'\in[k]}\alpha_{l'} (||x^l_{i_l} - x|| + \kappa_l ||a^l_{i_l} -a^l||) - \alpha_T (||x^T_{i_T} - x|| +  \sum_{l \in [k]}\kappa_l ||a^{T,l}_{i_T} -a^l||) \right)
\end{align*}
For notational convenience, we'll elide the subscript $i_l$ and $i_T$. Following the same argument as Lemma \ref{lem:conjugate-infimal-repr} and \ref{lem:conjugate-infimal-repr-fair}, we get
\begin{align*}
    &\sup_{b \in [0,1]} \sup_{(x, \{a_{l}\}_{l \in [k]})} \inf_{\substack{||q_l||_{*} \le \alpha_l, ||q'_l||_{*} \le \kappa_l \alpha_l \\||q_T||_{*}\le\alpha_T, ||q'_{T,l}||_{*}\le \kappa_{T,l} \alpha_T}} \langle b\theta, (x, \{a_{l}\}_{l \in [k]}) \rangle -f^*(b) - \sum_{l \in [k]} \langle q_l,  x^l \rangle - \langle q_T, x^T \rangle - \sum_{l \in [k]} \langle q'_l, a^l \rangle - \sum_{l \in [k]}\langle q'_{T,l}, a^{T,l} \rangle
\end{align*}


Applying Sion's minimax theorem to flip the order of $\sup$ and $\inf$, we get that if there doesn't exist $q, q'$ such that
\[
    b\theta[\cX] + \sum_{l \in [k]} q_l + q_T \neq 0
\]
and
\[
    b\theta[\cA_l] + q'_l + q'_{T,l} \neq 0
\]
the expression will evaluate to $\infty$. If not, we get that 
\begin{align*}
    &\sup_{b \in [0,1]} \inf_{\substack{||q_l||_{*} \le \alpha_l, ||q'_l||_{*} \le \kappa_l \alpha_l \\||q_T||_{*}\le\alpha_T, ||q'_{T,l}||_{*}\le \kappa_{T,l} \alpha_T}} -f^*(b) - \sum_{l \in [k]} \langle q_l,  x^l \rangle - \langle q_T, x^T \rangle - \sum_{l \in [k]} \langle q'_l, a^l \rangle - \sum_{l \in [k]}\langle q'_{T,l}, a^{T,l} \rangle \\
    &=\sup_{b \in [0,1]} \inf_{\substack{||q_l||_{*} \le \alpha_l, ||q'_l||_{*} \le \kappa_l \alpha_l \\||q_T||_{*}\le\alpha_T, ||q'_{T,l}||_{*}\le \kappa_{T,l} \alpha_T}} -f^*(b) + (g_1 \square \dots \square g_k \square g_T)(b\theta[\cX]) + \sum_{l \in [k]} (g'_1 \square g'_{T,l})(b\theta[\cA_l])
\end{align*}

\end{proof}

\subsection{Infimal Convolution of $k$ Linear Functions}
\begin{lemma}
\label{lem:inf-conv-k-anchor-affine}
Infimal convolution of linear functions with bounded norm domain is affine: 
\begin{align*}
    (g_1 \square \dots \square g_k)(\theta) = \begin{cases}\langle \gamma'_k, \theta \rangle + m'_k\quad\text{if $||\theta||_{*} \le \sum_{l \in [k]}\alpha_l$ }\\\infty \quad\text{otherwise}\end{cases}
\end{align*}
for some $\gamma'_k$ and $m'_k$ where $g_l(\theta) = \langle \gamma_l, \theta \rangle$ if $||\theta||_{*} \le \alpha_l$ and $\infty$ otherwise for each $l \in [k]$.
\end{lemma}
\begin{proof}
We will prove this by inducting on $k$. We have shown for $k=2$, the infimal convolution of linear functions is indeed affine with bounded norm domain in Lemma \ref{lem:inf-conv-affine}: 
\begin{align*}
    (g_1 \square g_2)(\theta) = \begin{cases}\langle \gamma'_2, \theta \rangle + m'_2 \quad\text{if $||\theta||_{*} \le \alpha_1 + \alpha_2$}\\ \infty \quad\text{otherwise}\end{cases}
\end{align*}
for some $\gamma'_2$ and $m'_2$. 

So suppose that for some $k > 2$ we have 
\begin{align*}
    (g_1 \square \dots  \square g_{k-1})(\theta) = \begin{cases}
         \langle \gamma'_{k-1}, \theta \rangle + m'_{k-1}\quad\text{if $||\theta||_{*} \le \alpha_1 + \alpha_2 + \dots + \alpha_{k-1}$}\\ \infty \quad\text{otherwise}
    \end{cases}
\end{align*}
for some $\gamma'_{k-1}$ and $m'_{k-1}$. For simplicity, we write $g'_{k-1}(\theta) = \langle \gamma'_{k-1}, \theta \rangle$ and $\alpha'_{k-1} = \sum_{l=1}^{k-1} \alpha_l$. In other words, \begin{align*}
    (g_1 \square \dots \square g_k)(\theta) = (g'_{k-1} \square g_k)(\theta) + m'_{k-1}.
\end{align*}

We can use Lemma \ref{lem:inf-conv-affine} to conclude that 
\begin{align*}
    (g'_{k-1} \square g_k)(\theta) = \begin{cases}\langle \gamma'_k, \theta \rangle + m_k \quad\text{if $||\theta||_{*} \le \alpha'_{k-1} + \alpha_k$ }\\\infty \quad\text{otherwise}\end{cases}.
\end{align*}

In other words, we have 
\begin{align*}
    (g_1 \square \dots \square g_k)(\theta) = \begin{cases}
         \langle \gamma'_{k}, \theta \rangle + m'_{k}\quad\text{if $||\theta||_{*} \le \sum_{l\ in [k] }\alpha_l$}\\ \infty \quad\text{otherwise}
    \end{cases}
\end{align*}
where $m'_k = m'_{k-1} + m_k$.
\end{proof}

Now, as before, we will evaluate the infimal convolution at $0$ and at a point where the norm constraints are tight as in Lemma \ref{lem:inf-conv-at-zero} and \ref{lem:inf-conv-tight}.

\begin{lemma}
\label{lem:inf-conv-k-tight}
Given $\overline{\theta}_{*}$ where $||\overline{\theta}_{*}||_{*} = 1$, we have 
\begin{align*}
    (g_1 \square \dots \square g_k)\left(\sum_{l\in[k]}\alpha_l \overline{\theta}_{*}\right) = \sum_{l \in [k]} \alpha_l \langle \gamma_l, \overline{\theta}_{*}\rangle.
\end{align*}
\end{lemma}
\begin{proof}
    As in Lemma \ref{lem:inf-conv-tight}, the only $(q_1, \dots, q_k)$ such that $||q_l||_{*} \le \alpha_l$ for each $l \in [k]$ and $\sum_{l \in [k]} q_l = \sum_{l \in [k]} \alpha_l \overline{\theta}_{*}$ is $(q_1, \dots, q_k) = (\alpha_1 \overline{\theta}_{*}, \dots, \alpha_k \overline{\theta}_{*})$. 
    
    Suppose not, meaning there exists different $(q'_1, \dots, q'_k)$ that satisfies the conditions. Without loss of generality, we choose the coordinate on which $q$ and $q'$ differ to be $k$ --- i.e. $q_k \neq q'_k$. Let's say $q'_l = q_l + \epsilon_l$ for every $l \in [k-1]$ and $q'_k = q_k - \sum_{l\in[k-1]} \epsilon_l$ where $\sum_{l\in[k-1]} \epsilon_l \neq 0$. In other words, there has to exist one $l' \in [k-1]$ such that $\epsilon_{l'} \neq 0$ because otherwise $(q_1, \dots, q_k) = (q'_1, \dots, q'_k)$.
    
    For any $l \in [k-1]$, Corollary \ref{cor:dual-norm-normal-vector} tells us that for any other $q'_l$ where $||q'_l||_{*} \le \alpha_l$, 
    \begin{align*}
        \langle v(\overline{\theta}_{*}), q_l + \epsilon_l \rangle &\le \langle v(\overline{\theta}_{*}), q_l \rangle\\
        \langle v(\overline{\theta}_{*}), \epsilon_l \rangle &\le 0.
    \end{align*}
    And for $l'$, we have a strict inequality as $q'_{l'} \neq q_{l'}$: 
    \begin{align*}
        \langle v(\overline{\theta}_{*}), q_{l'} + \epsilon_l \rangle &< \langle v(\overline{\theta}_{*}), q_{l'} \rangle\\
        \langle v(\overline{\theta}_{*}), \epsilon_{l'} \rangle &< 0.
    \end{align*}
    
   Then, we must have
   \begin{align*}
       ||q'_k||_{*} = \left\langle v(q'_k), q_k - \sum_{l \in [k-1]} \epsilon_l \right\rangle > \left \langle v(\overline{\theta}_{*}), q_k - \sum_{l \in [k-1]} \epsilon_l \right\rangle = \alpha_k - \sum_{l \in [k-1]}\langle v(\overline{\theta}_{*}), \epsilon_l \rangle > \alpha_k.
   \end{align*}
   
   Therefore, because $(\alpha_1 \overline{\theta}_{*}, \dots, \alpha_k \overline{\theta}_{*})$ is the only possible way of satisfying the conditions where $||q_l||_{*} \le \alpha_l$ for each $l \in [k]$ and $\sum_{l \in [k]} q_l = \sum_{l \in [k]} \alpha_l \overline{\theta}_{*}$, the infimal convolution evaluates to the following: 
   \begin{align*}
    (g_1 \square \dots \square g_k)\left(\sum_{l\in[k]}\alpha_l \overline{\theta}_{*}\right) = \sum_{l \in [k]} \alpha_l \langle \gamma_l, \overline{\theta}_{*}\rangle.
\end{align*}
\end{proof}

\begin{lemma}
\label{lem:inf-conv-k-zero}
$m'_k$ as defined in Lemma \ref{lem:inf-conv-k-anchor-affine} as the intercept of the infimal convolution of $k$ functions is recursively defined as
\[
    m'_k = m'_{k-1} - \alpha_k||\gamma'_{k-1} - \gamma_k||
\]
where $\gamma'_k$ is the slope of $(g_1 \square \dots \square g_k)(\theta)$ as defined in Lemma \ref{lem:inf-conv-k-anchor-affine}.
\end{lemma}
\begin{proof}
    From Lemma \ref{lem:inf-conv-k-anchor-affine}, we know that 
    \begin{align*}
         (g_1 \square \dots \square g_{k-1})(0)= g'_{k-1}(\theta) = \langle \theta, \gamma'_{k-1}\rangle + m'_{k-1}.
    \end{align*}
    
    Then we get
    \begin{align*}
        m'_k = (g'_{k-1} \square g_k)(0) &= \inf_{||q||_{*} \le \alpha_k} g'_{k-1}(q) + g_k(-q) \\ 
        &= m'_{k-1} + \inf_{||q||_{*} \le \alpha_k} \langle q, \gamma'_{k-1} - \gamma_k \rangle\\
        &=m'_{k-1} - \alpha_k||\gamma'_{k-1} - \gamma_k||
    \end{align*}
\end{proof}

As in Theorem \ref{thm:inf-conv-exact-slope}, by trying out the standard basis vectors scaled by $\sum_{l} \alpha_l$, we can calculate the slope exactly as the following:
\begin{lemma}
Each coordinate of $\gamma'_k$ is defined as:
    \[
        \gamma'_{k}[c] = \frac{\sum_{l \in [k]}\alpha_l\gamma_l[c]  - m'_k}{\sum_{l \in [k]} \alpha_k}.
    \]
\end{lemma}
\begin{proof}
    This is just an application of Theorem \ref{thm:inf-conv-exact-slope}.
    Due to the linearity of $(g_1 \square \dots \square g_k)(\theta)$, we can apply Lemma \ref{lem:inf-conv-k-tight} and \ref{lem:inf-conv-k-zero} to standard basis vector $e_c$ scaled by $\sum_{l\in [k]}\alpha_l$ for each coordinate $c$. More specifically, due to the linearity, we have for any $\overline{\theta}_{*}$, 
    \begin{align*}
        (g_1 \square \dots \square g_k)(b \overline{\theta}_{*}) = b \cdot s + m'_k.
    \end{align*}
    
    By using two points evaluated at $0$ and $\sum_{l \in [k]}\alpha_l \overline{\theta}_{*}$, we get the slope is 
    \begin{align*}
        s = \frac{\sum_{l \in [k]} \alpha_l \langle \overline{\theta}_{*}, \gamma_l \rangle - m'_k}{\sum_{l \in [k]} \alpha_l}.
    \end{align*}
    
    Trying out $\overline{\theta}_{*} = e_c$ for each coordinate $c$, we get
    \[ 
        \gamma'_k[c] = \frac{\sum_{l \in [k]}\alpha_l\gamma_l[c]  - m'_k}{\sum_{l \in [k]} \alpha_k}.
    \]
    
\end{proof}


==> unused_content.tex <==
\section{New Direction(s)}
Here's a setting that sounds a little bit more realistic. We have an auxiliary dataset that consists of feature vectors and protected attribute $S_a = \{(x_i,a_i)\}_{i=1}^{n_a}$ drawn from some distribution $\cP_A$ from which we try to learn the protected attribute predictor $h$.

And we have many different prediction tasks on which we want to use the above protected attribute predictor. For any prediction task, suppose we have some dataset $S = \{(x_i, y^t_i)\}_{i=1}^{n_p}$ drawn from $\cP_p$ from which we learn a predictor $f_p$. However, once we deploy the learned predictor $f_p$, the actual distribution is is some $\cPtest_p$ that might not be necessarily exactly $\cP_p$. 

Can we apply some robust optimization techniques that is better suited for this situation where you have these different distributions $\cP_a, \cP_p, \cPtest_p$ under some mild assumptions (e.g. $\cP_a$ and $\cPtest_p$ are pretty similar over $(x,a)$ and $\cP_p$ and $\cPtest_p$ are pretty similar over $(x,y)$)?  Here's one possible concrete problem. 
\begin{align*}
    \min_{\theta} \sup_{\cQtest \in B(\tP_{S_a}, \tP_{S_p}, r_a, r_p)} L_p(\theta, \cQtest) + \eta \cdot \Lfair(\theta, \cQtest).
\end{align*}
where 
\begin{enumerate}
    \item $r_a$: tolerance parameter for the proxy attribute prediction task
    \item $r_p$: tolerance parameter for prediction task $p$
    \item $\eta$: fairness penalty.  
    \item $\Lfair$: fairness loss
    \item $L_p$: prediction risk
    \item $B(\tP_{S_a}, \tP_{S_p}, r_a, r_p)=$\[\{\cQ \text{ over $(x,a,y)$}: \text{marginal distribution over $(x,a) \in B(\tP_{S_a}, r_a)$ , and marginal distribution over $(x,y) \in B(\tP_{S_p}, r_p)$}\}\]
\end{enumerate}
\newpage



\subsection{ADMM and AMA}
Here we describe how our optimization problem can be viewed as a problem where one can utilize Alternating Direction Method of Multipliers (ADMM) or Alternating Minization Algorithm (AMA). In fact, \cite{li2019first} show that instead of relying on off-the-shelf solvers such as YALMIP, ADMM with some modification (which we will describe a little later in this section) can enjoy a hundred-fold speedup in the case of distributionally logistic regression optimization problem whose problem structure is very similar to ours.

Consider the following optimization problem
\begin{align*}
    \min_{x,y} \quad &F(x,y) = f(x) + g(y) \\
    \text{s.t.} \quad &Ax = y
\end{align*}
where $f$ is a closed convex function that is strongly convex, $g$ is a closed convex function.

Now, define Augmented Lagrangian as 
\[
    \cL_\lambda(x,y, z) = f(x) + g(y) + \langle z, Ax-y\rangle + \frac{\lambda}{2}||Ax-y||^2_2
\]

\begin{algorithm}
    \caption{Alternating Minimization Algorithm (AMA)}
    \label{alg:AMA}
    \begin{algorithmic}
        \FOR{$t=1,\dots, T$}
            \STATE $x^{t+1} = \arg\min_{x} \cL_{0}(x, y^{t}, z^t)$\\
            \STATE $y^{t+1} = \arg\min_{y} \cL_{\lambda}(x^{t+1}, y^{t}, z^t)$\\
            \STATE $z^{t+1} = z^{t} + \lambda(Ax^{t+1} - y^{t+1})$
        \ENDFOR
    \end{algorithmic}
\end{algorithm}


\newcommand{\prox}{\text{Prox}}
We note that AMA is basically running a proximal gradient method in the dual space. More specifically, define the proximal operator as 
\[
    \prox_{\lambda f}(x) = \arg\min_{u} f(u) + \frac{\lambda}{2}||u-x||^2_2
\]
The corresponding dual problem is 
\[
    \max_{z} -f^*(-A^\top z) -g^*(z)
\]
and the proximal gradient descent with respect to this dual problem is
\[
    z^{t+1} = \prox_{\lambda g^*}(z^t + \lambda A \nabla f^*(-A^\top z^t)). 
\]
Using Moreau decomopsition (i.e. $x = \prox_h(x) + \prox_{h^*}(x)$), one can verify that this is exactly the same as AMA.

Another approach that one can use is ADMM which is very similar to AMA except for the $x$-update, it uses the augmented Lagrangian instead of the normal Lagrangian.

\begin{algorithm}
    \caption{Alternating Direction Method of Multipliers(ADMM)}
    \label{alg:ADMM}
    \begin{algorithmic}
        \FOR{$t=1,\dots, T$}
            \STATE $x^{t+1} = \arg\min_{x} \cL_{\lambda}(x, y^{t}, z^t)$\\
            \STATE $y^{t+1} = \arg\min_{y} \cL_{\lambda}(x^{t+1}, y^{t}, z^t)$\\
            \STATE $z^{t+1} = z^{t} + \lambda(Ax^{t+1} - y^{t+1})$
        \ENDFOR
    \end{algorithmic}
\end{algorithm}



\cj{TODO: Describe the relationship between ADMM and AMA.}
\cj{TODO: linear convergence and can be accelerated. Goldsten et al paper}

\cj{TODO: Describe our problem}

\cj{TODO: Find some upperbound on $\alpha_A$ and $\alpha_P$ like the ADMM for DRO paper. And argue we can do the similar binary search approach.}


\cj{Proximal Gradient Approach}
Then, fixing $\alpha_A$ and $\alpha_P$, our problem can be described as 
\[
\min_{\theta} f(\theta) + g(\theta)
\]
with 
\begin{align*}
    f(\theta) &= \frac{1}{n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \log(1+ \exp(-y^P_j \langle (x^P_j, a^A_i), \theta\rangle))\\
    g(\theta) &= \frac{1}{n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \max(y^P_j (x^P_j, a^A_i) - \alpha_P k_P, 0) + \infty \ind\left[||\theta_1 ||_{*} \le \alpha_A + \alpha_P, ||\theta_2||_{*} \le \kappa_A \alpha_A\right].
\end{align*}

Proximal gradient approach will be 
\[
    \theta^{t+1} = \prox_{\eta g}(\theta^t + \eta \nabla f(\theta^t)).
\]
\cj{I don't necessarily understand why the DRO optimization paper says the proximal gradient descent is not suited for this optimization problem?.}

We briefly discussed the approach used by \cite{li2019first}. 
They considered
\begin{align*}
    g_1(\beta) &= \frac{1}{n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \log(1+ \exp(-\beta)) + \frac{1}{2n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} (\beta - \alpha_P k_P)\\
    g_2(\beta) &= \frac{1}{2n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} |\beta - \alpha_P k_P|\\
    g(\beta) &= g_1(\beta) + g_2(\beta) = \frac{1}{n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \log(1+ \exp(-\beta)) + \frac{1}{n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \max(\beta - \alpha_P k_P, 0) \\
    f(\theta) &= \infty \ind\left[||\theta_1 ||_{*} \le \alpha_A + \alpha_P, ||\theta_2||_{*} \le \kappa_A \alpha_A\right].
\end{align*}
with the constraint $A \theta = \beta$ where each row of $A$ is $y^P_j \langle (x^P_j, a^A_i)$. Instead of directly applying ADMM as written in Algorithm \ref{alg:ADMM}, they have used linear approximation of $g_1$: $\hat{g}_1(\beta;\beta^t) = g_1(\beta^t) + \langle \nabla g_1(\beta^t) (\beta - \beta^t) \rangle$
\[
    \beta^{t+1} = \arg\min_\beta \hat{g}_1(\beta;\beta^t) + g_2(\beta) + f(\theta^{t+1}) + \langle z, A\theta^{t+1}-\beta\rangle + \frac{\lambda}{2}||A\theta^{t+1}-\beta||^2_2.
\]

\cj{Be careful about the assumption. We have that only one of the functions is strongly convex}
\begin{theorem}[ADMM and AMA's convergence rate]
\[
    F(w^*) - F(w^t) \le O\left(\frac{1}{t}\right)
\]
\end{theorem}

First-order approximation still gives us the above linear convergence, and there exists accelerated versions for which we get $O(\frac{1}{t^2})$.


\subsubsection{Range for $\alpha_A$ and $\alpha_P$}
\cj{Under construction}
As in \cite{li2019first}, let's write down the KKT conditions for our problem. To do so, we will slightly modify the problem and write

\begin{align*}
    \min_{\alpha_A, \alpha_P, \theta_1, \theta_2, \{s_{i,j}\}} &(\alpha_A r_A + \alpha_P r_P) + \frac{1}{n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \left(f(y^P_j\langle\theta, (x^A_i, a^A_i) \rangle) + s_{i,j}  \right) + \alpha_P M\\
    \text{s.t.}\quad & - s_{i,j}\le 0 \quad \forall i \in [n_A], j \in [n_P]\\
    &s_{i,j} - y^P_j\langle\theta, (\hat{x}_{i,j}, a^A_i) \rangle-\alpha_P\kappa_P \le 0 \quad \forall i \in [n_A], j \in [n_P]\\
    &||\theta_1||_{*} - \alpha_A - \alpha_P \le 0\\
    &||\theta_2|_{*} - \kappa_A \alpha_A \le 0\\
    &\alpha_P - \alpha_A \le 0
\end{align*}
where $M = -\frac{1}{n_A n_P} \sum_{i,j} ||x^A_i -x^P_j||$.


Now, let's use $w'_{ij}$ $w_ij$ as the dual variables for the first two constraints, and $h_1, h_2, h_3$ for the following constraints. 
Then, writing down the KKT condition for the stationary condition yields 
\begin{align*}
    \alpha_A&: r_A - h_1 - \kappa_A h_2  - h_3 = 0\\
    \alpha_P&: r_P + M - \kappa_P w_{ij} - h_1 + h_3 = 0\\
    \theta&: \frac{1}{n_A n_P} \sum_{i,j} \nabla_{\theta} f(y^P_j\langle\theta, (x^A_i, a^A_i) \rangle) - w_{ij}  y^P_j (\hat{x}_{i,j}, a^A_i) +   (h_1 \partial ||\theta_1||_{*}, h_2 \partial ||\theta_2||_{*}) = 0\\
    s_{ij}&: \frac{1}{n_A n_P} - w'_{ij}+w_{ij} = 0.
\end{align*}

Multiplying both sides by $\theta$, we get
\begin{align*}
    0 &= \frac{1}{n_A n_P} \sum_{i,j} \theta \nabla_{\theta} f(y^P_j\langle\theta, (x^A_i, a^A_i) \rangle) - w_{ij}  y^P_j (\hat{x}_{i,j}, a^A_i) +   \theta (h_1 \partial ||\theta_1||_{*}, h_2 \partial ||\theta_2||_{*})
\end{align*}



Then, we get 
\begin{align*}
    0 \le \frac{1}{n_A n_P} \sum_{i,j} \theta \nabla_{\theta} f(y^P_j\langle\theta, (x^A_i, a^A_i) \rangle) - w_{ij}  y^P_j (\hat{x}_{i,j}, a^A_i)    
\end{align*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Optimization}



\iffalse
\begin{lemma}
\begin{align*}
    (g_1 \square g_2 \square g_3)(0) = \left|\left|\frac{\alpha_1 \gamma_1 + \alpha_2 \gamma_2}{\alpha_1 + \alpha_2} + \gamma_3 \right|\right| + \alpha_2\left(\frac{\alpha_3  || \gamma_1 - \gamma_2|| }{\alpha_1 + \alpha_2} - || \gamma_1 - \gamma_2||\right)
\end{align*}
where $\alpha_1 \ge \alpha_2 \ge \alpha_3$.
\end{lemma}
\begin{proof}
Because the infimal convolution of linear functionsw with bounded norm domain is affine from Lemma \ref{lem:inf-conv-k-anchor-affine}, we must have that \[
    (g_1 \square \dots \square g_k)(b \overline{\theta}_{*}) = \langle \gamma, b\overline{\theta}_{*}\rangle + m.
\]
 
From Theorem \ref{thm:inf-conv-closed-fo}, we know that 
\[
    (g_1 \square g_2)(b \overline{\theta}_{*})= \frac{\langle \overline{\theta}_{*}, \alpha_1 \gamma_1 + \alpha_2 \gamma_2 \rangle + \alpha_2 || \gamma_1 - \gamma_2||}{\alpha_1 + \alpha_2}
         \cdot b - \alpha_2 || \gamma_1 - \gamma_2||. 
\]

Then, we have
\begin{align*}
    ((g_1 \square g_2) \square g_3)(0) &= \inf_{||q||_{*} \le \alpha_3} (g_1 \square g_2)(q) + g_3(-q)\\
    &=\inf_{||q||_{*} = \alpha_3} (g_1 \square g_2)(\alpha_3\overline{q}_{*}) + g_3(-q)\\
    &=\inf_{||q||_{*} = \alpha_3} \frac{\langle \overline{q}_{*}, \alpha_1 \gamma_1 + \alpha_2 \gamma_2 \rangle + \alpha_2 || \gamma_1 - \gamma_2||}{\alpha_1 + \alpha_2}
         \cdot \alpha_3 - \alpha_2 || \gamma_1 - \gamma_2|| - \langle \gamma_3, q \rangle \\
    &= \inf_{||q||_{*} = \alpha_3} \langle q, \frac{\alpha_1 \gamma_1 + \alpha_2 \gamma_2}{\alpha_1 + \alpha_2} - \gamma_3 \rangle + \alpha_2\left(\frac{\alpha_3  || \gamma_1 - \gamma_2|| }{\alpha_1 + \alpha_2} - || \gamma_1 - \gamma_2||\right)\\
    &=\left|\left|\frac{\alpha_1 \gamma_1 + \alpha_2 \gamma_2}{\alpha_1 + \alpha_2} - \gamma_3 \right|\right| + \alpha_2\left(\frac{\alpha_3  || \gamma_1 - \gamma_2|| }{\alpha_1 + \alpha_2} - || \gamma_1 - \gamma_2||\right)
\end{align*}
The second equality follows from the fact $(g_1 \square g_2)$ and $g_3$ are linear, meaning it's a linear optimization over a convex set and that the optimal solution in that case happens at the boundary of the set. 
\end{proof}
\fi


\newpage
%%%%%%%%% THINGS BELOW THIS POINT SHOULD BE TAKEN OUT OF THE MAIN BODY %%%%%%%%%%
\section{$\sup_{x,a}$}

\begin{align*}
    &\sup_{(x,a)} h(\theta, (x, a)) - \alpha_A ||x^A_i - x||  -  \alpha_P ||x^P_j - x|| - \alpha_M || a^A_i - a||\\
    &=\sup_{(x,a)} \sup_{b \in [0,1]} \langle b\theta, (x,a) \rangle  - f^*(b) - \alpha_A ||x^A_i - x||  -  \alpha_P ||x^P_j - x||- \alpha_M || a^A_i - a||\\
    &= \sup_{b \in [0,1]} \sup_{(x,a)} \langle b\theta, (x,a) \rangle  - f^*(b) - \sup_{||q_1||_{*} \le \alpha_A}\langle q_1, x^A_i - x \rangle -  \sup_{||q_2||_{*} \le \alpha_P}\langle q_2, x^P_j - x\rangle- \sup_{||q_3||_{*}\le \alpha_M} \langle q_3, a^A_i - a\rangle\\
    &=  \sup_{b \in [0,1]} \sup_{(x,a)} \langle b\theta, (x,a) \rangle  - f^*(b) - \sup_{||q_1||_{*} \le \alpha_A}\langle (q_1, \xi_1), (x^A_i,a) - (x,a) \rangle -  \sup_{||q_2||_{*} \le \alpha_P}\langle (q_2, \xi_2), (x^P_j,a) - (x,a)\rangle \\
    &- \sup_{||q_3||_{*}\le \alpha_M} \langle (0,q_3), (0,a^A_i) - (x,a)\rangle\\
    &=  \sup_{b \in [0,1]} \sup_{(x,a)} \inf_{\substack{||q_1||_{*}\le \alpha_A,\\ ||q_2||_{*}\le \alpha_P, ||q_3||_{*} \le \alpha_M}} \langle b\theta, (x,a) \rangle  - f^*(b) - \langle (q_1, \xi_1), (x^A_i,a) - (x,a) \rangle - \langle (q_2, \xi_2), (x^P_j,a) - (x,a)\rangle \\
    &-\langle (0,q_3), (0,a^A_i) - (x,a)\rangle\\
    &= \sup_{b \in [0,1]} \sup_{(x,a)}  \inf_{\substack{||q_1||_{*}\le \alpha_A,\\ ||q_2||_{*}\le \alpha_P, ||q_3||_{*} \le \alpha_M}} \langle b\theta + (q_1, \xi_1) + (q_2,\xi_2) + (0,q_3), (x,a) \rangle  - f^*(b) - \langle (q_1, \xi_1), (x^A_i,a) \rangle - \langle (q_2, \xi_2), (x^P_j,a)\rangle\\
    &-\langle q_3, a^A_i\rangle\\
\end{align*}    

Now because everything is linear, Sion's theorem holds allowing us to swap $\inf$ and $\sup$:
\begin{align*}
    &= \sup_{b \in [0,1]}  \inf_{\substack{||q_1||_{*}\le \alpha_A,\\ ||q_2||_{*}\le \alpha_P}} \sup_{x}  \langle b\theta + (q_1, \xi_1) + (q_2,\xi_2) \rangle  - f^*(b) - \langle (q_1, \xi_1), (x^A_i,a) \rangle - \langle (q_2, \xi_2), (x^P_j,a)\rangle -\langle q_3, a^A_i\rangle.
\end{align*}
Note that unless $b\theta + (q_1, \xi_1) + (q_2, \xi_2) + (0, q_3) = 0$, $x$ can be chosen arbitrarily big. Also, if $\theta + (q_1, \xi_1) + (q_2, \xi_2) + (0,q_3) \neq 0$, then $b$ can be chosen to be 1. Therefore, if there doesn't exist $(q_1, \xi_1)$, $(q_2,\xi_2)$, and $q_3$ such that $\theta + (q_1, \xi_1) + (q_2, \xi_2) + (0,q_3) \neq 0$, everything evaluates to $\infty$. Since we are allowed to choose $\xi_1$ and $\xi_2$ arbitrarily, let's choose $\xi_1 = 0$ and $\xi_2 = 0$. Then, the only way for $\theta + (q_1, \xi_1) + (q_2, \xi_2) + (0,q_3) = 0$, we have to set $q_3 = -\theta[n+1:n+d]$ and we need to have $||\theta[n+1:n+d]||_{*} \le \alpha_M$. Now, we further simplify the expression.


\begin{align*}
    &= \sup_{b \in [0,1]} - f^*(b) \\
    &+ \inf_{\substack{||q_1||_{*}\le \alpha_A,\\ ||q_2||_{*}\le \alpha_P}, ||q_3||_{*} \le \alpha_M} \begin{cases}
          - \langle (q_1, \xi_1), (x^A_i,-a) \rangle - \langle (q_2, \xi_2), (x^P_j,-a)\rangle - \langle q_3, a^A_i\rangle &\quad\text{if $b\theta + (q_1, \xi_1) + (q_2, \xi_2) +(0,q_3)= 0$}\\
         \infty &\quad\text{otherwise}
    \end{cases}\\
    &= \langle \theta[n+1:n+d], a^A_i \rangle + \sup_{b \in [0,1]} - f^*(b) + \inf_{\substack{||q_1||_{*}\le \alpha_A,\\ ||q_2||_{*}\le \alpha_P}} \begin{cases}
          - \langle q_1, x^A_i \rangle - \langle q_2, x^P_j \rangle &\quad\text{if $b\theta[1:n] + q_1 + q_2 = 0$}\\
         \infty &\quad\text{otherwise}
    \end{cases}\\
    &= \langle \theta[n+1:n+d], a^A_i \rangle + \sup_{b \in [0,1]} - f^*(b) + (g^i_1 \square g^j_2)(-b\theta[1:n])
\end{align*}

\section{$k$-anchor case}
The primal problem is 
\begin{align}
\begin{split}
     \sup_{\pi^{a,y}_{i,j}} \quad&  \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \sum_{l=1}^{n_T} \sum_{y \in \cY}\int \ell(\theta, (x, a, y))  \pi^{y}_{i,j, l}(dx, da)\\
    \text{s.t.} \quad& \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{l=1}^{n_T} \sum_{y \in \cY}\int d_A^{i}(x,a)  \pi^{y}_{i,j, l}(dx, da) \le r_A\\
    \quad& \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{l=1}^{n_T} \sum_{y \in \cY}\int d_P^{j}(x,y)  \pi^{y}_{i,j, l}(dx, da) \le r_P \\
    \quad& \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{l=1}^{n_T} \sum_{y \in \cY}\int d_T^{l}(x,a,y)  \pi^{y}_{i,j, l}(dx, da) \le r_T \\
    \quad& \sum_{j=1}^{n_P} \sum_{l=1}^{n_T} \sum_{y \in \cY} \int \pi^{y}_{i,j,l}(dx, da) = \frac{1}{n_A} \quad \forall i \in [n_A]\\
    \quad& \sum_{i=1}^{n_A} \sum_{l=1}^{n_T} \sum_{y \in \cY} \int  \pi^{y}_{i,j,l}(dx, da)  = \frac{1}{n_P} \quad \forall j \in [n_P]\\
    \quad& \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \sum_{y \in \cY} \int  \pi^{y}_{i,j,l}(dx, da)  = \frac{1}{n_T} \quad \forall l \in [n_T]
\end{split}
\label{eqn:joint-transport-primal}
\end{align}

Corresponding dual problem is then
\begin{align}
\begin{split}
    &\inf_{\substack{\alpha_A, \alpha_P, \alpha_T \\ \{\beta_{i}\}_{i \in [n_A]}, \{\beta'_j\}_{j \in [n_P]}, \{\beta''_l\}_{l \in [n_T]}}} \quad \alpha_A r_A + \alpha_P r_P + \alpha_T r_T + \frac{1}{n_A}\sum_{i\in [n_a]} \beta_{i} + \frac{1}{n_P} \sum_{j \in [n_P]} \beta' + \frac{1}{n_T} \sum_{l \in [n_T]}  \beta''_l \text{such that}\\
    &\sup_{(x,a)} \left(\ell(\theta, (x, a, y)) - \alpha_A d^i_A(x,a)  - \alpha_P d^j_P(x,y) - \alpha_T d^l_T(x,a,y) \right) - \beta_{i} - \beta'_j -\beta''_l \le 0 \quad i \in [n_A], j \in [n_P], l \in [n_T], y \in \cY
\end{split}
\label{eqn:joint-transport-dual}
\end{align}





\section{Chris's playground}
\subsection{Fairness}
\cj{Actually try out all possibilities for the marginal distribution $\Pr(a, Y)$ and solve the inner optimization according to that fixed $\Pr(a,y)$. Among them, choose the worst one. }
\begin{align}
\begin{split}
     \sup_{\pi^{a,y}_{i,j}, \gamma} \quad&  \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \sum_{a \in A} \sum_{y \in \cY}\int \ell(\theta, (x, a, y))  \pi^{a,y}_{i,j}(dx)\\
    \text{s.t.} \quad& \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{a \in A} \sum_{y \in \cY}\int d_A^{i}(x,a)  \pi^{a,y}_{i,j}(dx) \le r_a\\
    \quad& \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{a \in A} \sum_{y \in \cY}\int d_P^{j}(x,y)  \pi^{a,y}_{i,j}(dx) \le r_P \\
    \quad& \sum_{j=1}^{n_P}\sum_{a \in A} \sum_{y \in \cY} \int \pi^{a,y}_{i,j}(dx) = \frac{1}{n_A} \quad \forall i \in [n_A]\\
    \quad& \sum_{i=1}^{n_A}\sum_{a \in A} \sum_{y \in \cY} \int  \pi^{a,y}_{i,j}(dx)  = \frac{1}{n_P} \quad \forall j \in [n_P]\\
    \quad& \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{a \in A} \sum_{y \in \cY}\int \ind[a=1, y=1]  \pi^{a,y}_{i,j}(dx) = \gamma_{1,1} \\
\end{split}
\end{align}

\begin{align}
\begin{split}
    &\inf_{\substack{\alpha_A, \alpha_P, \\ \{\beta_{i}\}_{i \in [n_A]}, \{\beta'_j\}_{j \in [n_P]}}} \quad \alpha_A r_A + \alpha_P r_P + \frac{1}{n_A}\sum_{i\in [n_A]} \beta_{i} + \frac{1}{n_P} \sum_{j \in [n_P]} \beta'\\
    &\text{such that} \quad \\
    &\sup_{x} \ell(\theta, (x, a, y)) - \alpha_A d^i_A(x,a)  -  \alpha_P d^j_P(x,y) - \beta_{i} - \beta'_j \le 0 \quad i \in [n_A], j \in [n_P], a \in \cA, y \in \cY
\end{split}
\end{align}

\begin{align*}
    \Lagr(\pi, \alpha_A, \alpha_P, \{\beta_{i,j}\}_{i,j}) &= \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{a \in A} \sum_{y \in \cY}\int \ell(\theta, (x, a, y))  \pi^{a, y}_{i,j}(dx))\\
    &+ \alpha_A \left(r_A - \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{a \in \cA} \sum_{y \in \cY}\int d^i_A(x,a)  \pi^{a,y}_{i,j}(dx)  \right) \\
    &+ \alpha_P \left(r_P - \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{a \in \cA} \sum_{a \in \cY} \int d^j_P(x,y)  \pi^{a,y}_{i,j}(dx)  \right)\\
    &+ \sum_{i=1}^{n_A} \beta_{i} \left(\frac{1}{n_A}- \sum_{j=1}^{n_P}\sum_{a \in \cA} \sum_{y \in Y} \int \pi^{a,y}_{i,j}(dx) \right)\\
    &+ \sum_{j=1}^{n_P} \beta'_{j} \left(\frac{1}{n_P} - \sum_{i=1}^{n_A}\sum_{a \in \cA} \sum_{y \in Y} \int \pi^{a,y}_{i,j}(dx) \right)\\
    &+ \omega_{1,1} \left( \gamma_{1,1} - \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{a \in A} \sum_{y \in \cY}\int \ind[a=1, y=1]  \pi^{a,y}_{i,j}(dx)\right)
\end{align*}

\begin{align*}
    &\Lagr(\pi, \alpha_A, \alpha_P, \{\beta_{i}\}, \{\beta'_{j}\}\})\\
    &= \sum_{i=1}^{n_A}\sum_{j=1}^{n_P} \sum_{a \in \cA} \sum_{y \in \cY}\int \left(\ell(\theta, (x, a, y)) - \alpha_A d^i_A(x,a) -  \alpha_P d^j_P(x,y) - \beta_i  - \beta'_j - \omega_{1,1} \ind[a=1, y=1] \right) \pi^{y, a}_{i,j}(dx)+ \omega_{1,1}\gamma_{1,1}\\
    &+ \alpha_A r_A + \alpha_P r_P + \frac{1}{n_A} \sum_{i=1}^{n_A} \beta_i + \frac{1}{n_P} \sum_{j=1}^{n_P} \beta'_j. 
\end{align*}

\subsection{Possibility of Protected Attribute Predictor for Many Tasks}
\cj{It would be cool, if it's possible for us to come up with $h$ that is approximately optimal for any $f \in \cF$ so that it can be used generally for any prediction task. It most likely won't be the case..}
\cj{A lot of the previous work shows that the min-max problem can be solved and shows how to actually construct the worst case distribution. I'm going to try to dig deeper into the details of previous work in this approach. }
Can we be task-agnostic and build a $h$ by looking at the optimization problem below: 
\begin{align*}
    \sup_{\theta} \sup_{\cQtest \in B(\tP_{S_a}, r_a)}  \Lfair(\theta, \cQtest).
\end{align*}

\subsection{Lowerbound}
Unless we assume there is some `commonality' between the protected attributes dataset $S_A$ and the prediction task dataset $S_p$, we need to show that it is impossible the above problem. 

I envision that this commonality can be expressed in terms of either (1) some common dataset $\{(x,a,y)\}$ or (2) some distribution distance between $S_A$ and $S_p$. It's just a little confusing how to describe the distribution distance between $S_A$ and $S_p$ when they only share $x$'s and not $a$ or $y$'s -- it might be possible to just describe the distance between the marginal distribution over the $x$'s?   
\begin{table}[h!]
    \begin{minipage}{.4\textwidth}
      \centering
      \begin{tabular}{cc}
        \toprule $x$ & $a$ \\ \midrule 
        1 & 0\\
        1 & 1\\
        \bottomrule
      \end{tabular}
      \caption{$S_a$}
    \end{minipage}
    \begin{minipage}{.4\textwidth}
      \centering
      \begin{tabular}{cc}
        \toprule $x$ & $y$ \\ \midrule 
        1 & 0\\
        1 & 1\\
        \bottomrule
      \end{tabular}
      \caption{$S_p$}
    \end{minipage}
  \end{table}



Possible ways to ``stitch'' these two datasets together such that the marginal distributions stay the same:

\begin{table}[h!]
    \begin{minipage}{.33\textwidth}
      \centering
      \begin{tabular}{ccc}
        \toprule $x$ & $a$ & $y$ \\ \midrule 
        1 & 0 & 0 \\
        1 & 0 & 1 \\
        1 & 1 & 0 \\
        1 & 1 & 1
    \end{tabular}
    \end{minipage}
    \begin{minipage}{.33\textwidth}
      \centering
      \begin{tabular}{ccc}
        \toprule $x$ & $a$ & $y$ \\ \midrule 
        1 & 0 & 0 \\
        1 & 1 & 1 \\
    \end{tabular}
    \end{minipage}
    \begin{minipage}{.33\textwidth}
      \centering
      \begin{tabular}{ccc}
        \toprule $x$ & $a$ & $y$ \\ \midrule 
        1 & 0 & 1 \\
        1 & 1 & 0 \\
    \end{tabular}
    \end{minipage}
    \caption{Possible joint distributions with the same marginal distribution as $S_a$ and $S_p$}
  \end{table}



Suppose we can boil the optimization problem down to the following problem\cj{TODO: this can be made into a lemma possibly.}
\[
L_p(\theta, S_p) + \Lfair(\theta, S_a),
\]
such as when $\Lfair(\theta, S_a) = \left\vert \Pr_{\tP_{S_a}}[f_p(x ; \theta) = 1 |a =0] - \Pr_{\tP_{S_a}}[f_p(x;\theta) = 1 |a =1] \right\vert $ is measuring the difference in positive rates (i.e. statistical parity); in other words, the unfairness does not require access to $y$ values when measuring the fairness risk. Then, the above stitching problem disappears as all three joint distributions have the same $\Lfair$. 

However, a lot of fairness risks cannot be simply evaluated on the marginal distributions over $(x,a)$. So, suppose we are focusing on difference in false positive rates (this should be equivalent to trying to achieve equal opportunity). But even in this case, DRO will simply choose the worst-case distribution, so does it actually matter which joint distribution we optimize over? Actually, it's possible that the range of unfairness risk can be vastly different. So, the kind of theorem (or lemma) statement we are looking for tries to analyze the range in fairness risk when focusing on $B(\tP_{S_a}, \tP_{S_p}, r_A, r_p)$. What we can hope to show is that if we have a third distribution that somewhat anchors both the protected attribute dataset and the prediction task dataset, this range in fairness risk can be much smaller. Maybe, it'll be hard to quantitatively bound this risk, but maybe, one can actually quantitiavely bound how much smaller the feasible region becomes? 

One question: do we need to worry about some triangle inequality once we introduce a third joint dataset? More specifically, previously, we were looking at a worst case joint distribution that is in the intersection of the $r_A$-ball of the Wasserstein ball around $\tP_{S_A}$ and $r_p$-ball of the Wasserstein ball around $\tP_{S_p}$. But now we are looking at the intersection of three balls where the third ball is centered at the joint dataset. Need to understand the metric structure of Wasserstein distance a little more.

Here let me try to write down the dual of the optimization problem which usually simplifies the original optimization in the case of the Wasserstein distance. 

Remember that given $S_p = \{(x^p_i, y^p_i)\}_{i=1}^{n_p}$ and $S_a = \{x^A_i, y^a_i\}_{i=1}^{n_A}$, the primal optimization problem is to solve
\begin{figure}[h!]
\begin{align*}
    \min_{\theta}  \sup_{Q} \quad& L_p(\theta, Q) + \eta \cdot \Lfair(\theta, Q)\\
    \text{s.t.} \quad& Q(X,A) \in B(\tP_{S_a}, r_a)\\
    &Q(X,Y) \in B(\tP_{S_p}, r_p),
\end{align*}
    \caption{Non-joint optimization problem}
    \label{fig:non-joint-opt}
\end{figure}
where $Q(X,A)$ refers to $Q$'s marginal distribution over $(x,a)$ and similarly $Q(X,Y)$ the marginal distribution over $(x,y)$.

If we are also given some $S_d = \{(x^d_i, a^d_i, y^d_i)\}_{i=1}^{n_d}$
\begin{figure}[h!]
    \begin{align*}
        \min_{\theta}  \sup_{Q} \quad& L_p(\theta, Q) + \eta \cdot \Lfair(\theta, Q)\\
        \text{s.t.} \quad& Q(X,A) \in B(\tP_{S_a}, r_a)\\
        &Q(X,Y) \in B(\tP_{S_p}, r_p)\\
        &Q \in B(\tP_{S_d}, r_d)
    \end{align*}
    \caption{Joint optimization problem}
    \label{fig:joint-opt}
\end{figure}

Actually, I think the problem here is exactly captured by \cite{kallus2021assessing} where they study $\{Q: Q(X,A) \in B(\tP_{S_a}, 0), Q(X,Y) \in B(\tP_{S_p}, 0)\}$. One useful tool they use is Fr\'{e}chet-Hoeffding Inequality that characterizes the coupling set exactly. They give a lower and upper bound on $\Lfair$ (exactly? I believe) for any given $\theta$.  
\section{Chris's Sandbox Below}
\subsection{Exercise: Duality for Distributionally Robust Logistic Regression}
Now, just as an exercise in deriving the duality, let's try to find the dual to the following distributionally robust logistic regression\footnote{I'm essentially copying over the proof of \cite{shafieezadeh2015distributionally}}: given $S = \{(x_i,y_i)\}_{i=1}^n$ where $y_i \in \{\pm 1\}$,


\begin{align}
    \min_{\theta} \sup_{Q: Q \in B(\tP_{S}, r)} L_p(\theta, Q) \label{opt:dr-logistic-regression}
\end{align}
where $L_p(\theta, Q) = \E_{z \sim Q}[\ell_\theta(z)]$ and $\ell_\theta((x,y)) = \log(1 + \exp(-y \langle \theta, x \rangle))$ is the logloss function and the the prediction made with parameter $\theta$ is $\Pr(y |x, \theta) = \frac{1}{1 + \exp(-y \langle \theta, x \rangle)}$. The metric used for the Wasserstein distance is $d((x,y), (x',y')) = || x-x'|| + \kappa |y-y'|/2$.

Using the fact that the dual of $f^*_\theta$ must be $f_\theta$ because it's convex and lower semi-continuous, one can easily show the following:
\begin{lemma}[Lemma 1, \cite{shafieezadeh2015distributionally}]
\label{lem:convex_conj_duality}
Given a $f(\theta, x) = \log(1 + \exp(-y \langle \theta, x \rangle))$ that is convex in $x$ where $x,\theta \in \R^d$, we have
\[
\sup_{x \in \R^d} f(\theta, x) -\lambda || \hat{x} - x|| = 
\begin{cases}
     f(\theta, \hat{x}) & ||\theta||_{*} \le \lambda\\
    -\infty &\text{otherwise}
\end{cases}
\]
for every $\lambda > 0$, where $||\cdot||_{*}$ is the dual norm of $|| \cdot ||$ i.e. $||\cdot||_{*} = \sup_{|| x|| \le 1} \langle \theta, x\rangle$. 
\end{lemma}

\begin{theorem}[Strong Duality of DR logistic regression]
Optimization problem \eqref{opt:dr-logistic-regression} is equivalent to 
\begin{align*}
    \min_{\theta, \lambda, s_i} \quad& \lambda r + \frac{1}{n} \sum_{i=1}^n s_i \\
    \text{such that} \quad& \ell_\theta((x_i, y_i)) \le  s_i \quad \forall i \in [n]\\
    \quad& \ell_\theta((x_i, -y_i)) - \lambda \kappa \le s_i \quad i\in [n] \\
    \quad&||\theta||_{*} \le \lambda
\end{align*}
\end{theorem}
\begin{proof}
First, note that because the Wasserstein distance is with respect to the empirical distribution which is a discrete uniform distribution over $\{(x_i, y_i)\}_{i=1}^n$, we will write $Q^i(dz)$ to denote the conditional marginal distribution where we conditioned on $(x_i, y_i)$ for some joint distribution $\Pi$ over $((x_i, y_i), (x,y))$ -- i.e. $Q^i(z) = \Pi((x_i,y_i), z)$.

The objective value in the primal optimization problem is equivalent to 
\begin{align*}
    \sup_{Q^{i}} \quad& \frac{1}{n} \sum_{i=1}^n \int \ell_\theta(z) Q^i(dz)   \\
    \text{such that} \quad& \frac{1}{n} \sum_{i=1}^n \int d((x_i, y_i), z) Q^i(dz) \le r \\
    \quad& \int Q^i(dz) = 1 \quad\forall i \in [n].
\end{align*}
Essentially, the sup is over all possible conditional marginal distribution $Q^i$. For simplicity, let's write $d^i(z) = d((x_i, y_i), z)$

By further dividing the conditional marginal distribution $Q^i$ into $Q^i_{+1}$ and $Q^i_{-1}$ depending on the label $y$, the above optimization problem is equivalent to:
\begin{align*}
    \sup_{Q^{i}} \quad& \frac{1}{n} \sum_{i=1}^n \int \ell_\theta((x,+1)) Q_{+1}^i(dz) + \int \ell_\theta((x,-1)) Q_{-1}^i(dz)  \\
    \text{such that} \quad& \frac{1}{n} \sum_{i=1}^n \left(\int d((x_i, y_i), (x,+1)) Q_{+1}^i(dx)\right) + \left(\int d((x_i, y_i), (x,-1)) Q_{-1}^i(dx)\right) \le r \\
    \quad& \int Q_{+1}^i(dz) + Q_{-1}^i(dz) = 1 \quad\forall i \in [n].
\end{align*}



Consider the Lagrangian of the above optimization problem:
\begin{align*}
&\mathcal{L}(\{\alpha_i\}, \beta) \\
&= \sup_{\{Q^i_{\pm 1}\}_i} \frac{1}{n} \sum_{i=1}^n \int \left(\ell_\theta(x,+1) - \beta d^i(x,+1) - n \alpha_i  \right) Q_{+1}^i(dz) + \int \left(\ell_\theta(x,-1) - \beta d^i(x,-1) - n \alpha_i  \right) Q^i(dz)\\
&+ \sum_{i=1}^n \alpha_i + r \beta.
\end{align*}

\cj{Two options: fenchel duality or minmax = max min proof. Let me try to the fenchel duality proof here.}
Note that we cannot have any $z^*$ such that for any $i \in [n]$,
\[
    \ell_\theta(z^*) - \beta d^i(z^*) - n \alpha_i > 0.
\]
Otherwise, the Lagrangian will be unbounded as we can put all the mass in the neighborhood around $z^*$, and due to continuity of the above value, $\int \left(\ell_\theta(z) - \beta d^i(z) - n \alpha_i  \right) Q^i(dz)$ will be $\infty$. And this contradicts the strong duality -- see these \href{https://www.math.cmu.edu/~mthorpe/OTNotes}{lecture notes} for more detail from which we can also find appropriate references, but anyway, we essentially need a minmax theorem to hold here for this.

Therefore, we have for all $z$,
\[
    \ell_\theta(z) - \beta d^i(z) - n \alpha_i \le 0.
\]
In fact, the primal optimal solution $\{Q^i\}_i$ will satisfy
\[
    \sup_{Q_i} \frac{1}{n} \sum_{i=1}^n \int \left(\ell_\theta(z) - \beta d^i(z) - n \alpha_i  \right) Q^i(dz)  + \sum_{i=1}^n \alpha_i + r \beta = \sum_{i=1}^n \alpha_i + r \beta
\]
with the following that holds for all $i \in [n]$
\[
    \int \left(\ell_\theta(z) - \beta d^i(z) - n \alpha_i  \right) Q^i(dz) = 0.
\]
\cj{The end of the duality proof here.}
Therefore, the dual objective is
\begin{align*}
    \min_{\{\alpha_i\}_i, \beta} \quad& \sum_{i=1}^n \alpha_i + r \beta \\
    \text{such that}\quad& 
    \sup_{x} \ell_\theta(x, +1) - \beta d^i(x,+1) - n \alpha_i \le 0 \quad \forall i \in [n]\\
    &\sup_{x} \ell_\theta(x, -1) - \beta d^i(x,-1) - n \alpha_i \le 0 \quad \forall i \in [n].
\end{align*}

Actually, expanding out the $d^i$ terms, we get
\begin{align*}
    \min_{\{\alpha_i\}_i, \beta} \quad& \sum_{i=1}^n \alpha_i + r \beta \\
    \text{such that}\quad& 
    \sup_{x} \ell_\theta(x, +1) - \beta \left(||x_i - x|| - \frac{\kappa}{2}|1 - y_i| \right)  \le n \alpha_i \quad \forall i \in [n]\\
    &\sup_{x} \ell_\theta(x, -1) - \beta \left(||x_i - x|| - \frac{\kappa}{2}|1 + y_i| \right)\le n \alpha_i \quad \forall i \in [n].
\end{align*}



Now, we can apply Lemma \ref{lem:convex_conj_duality} to $\sup_{x} \ell_\theta(x, -1) - \beta ||x_i - x|| $ as $\ell_\theta(x,-1)$ is convex. Therefore, we are left with the following optimization problem:
\begin{align*}
    \min_{\{\alpha_i\}_i, \beta, \theta} \quad& \sum_{i=1}^n \alpha_i + r \beta \\
    \text{such that}
    \quad& \ell_\theta(x_i, +1) - \frac{\kappa}{2}|1 - y_i|   \le n \alpha_i \quad \forall i \in [n]\\
    &\ell_\theta(x_i, -1) - \frac{\kappa}{2}|1 + y_i|   \le n \alpha_i \quad \forall i \in [n]\\
    \quad& || \theta||_{*} \le \beta.
\end{align*}
\end{proof}



\subsection{Dual for our problem}
For now, let's even ignore the fairness risk. The objective we are interested in is
after\cj{Discuss possible new notation for marginalizing some joint distribution.}
\begin{align*}
    \sup_{Q} \quad&  \frac{1}{n_p}\sum_{i=1}^{n_p} \int \ell_p(\theta, (x, a, y))  \Pi_p((x^p_i, y_i), (dx, da, dy)) \\
    \text{s.t.} \quad& \frac{1}{n_a} \sum_{i=1}^{n_a} \int d_a((x^A_i, a_i), (x,a)) \Pi_a((x^A_i, a_i), (dx, da, dy)) \le r_a\\
    \quad& \frac{1}{n_p}\sum_{i=1}^{n_p}\int d_p((x_i, y_i), (x,y)) \Pi_p((x^p_i, y_i), (dx, da, dy)) \le r_p\\
    \quad& \frac{1}{n_a}\sum_{i=1}^{n_a} \Pi_a((x^A_i, a_i), (x, a, y)) \le \frac{1}{n_p}\sum_{i=1}^{n_p} \Pi_p((x^p_i, y_i), (x, a, y)) \quad \forall x, a, y\\
    \quad& \frac{1}{n_p}\sum_{i=1}^{n_p} \Pi_p((x^p_i, y_i), (x, a, y)) \le \frac{1}{n_a}\sum_{i=1}^{n_a} \Pi_a((x^A_i, a_i), (x, a, y)) \quad \forall x, a, y
\end{align*}
The last two inequalities are to enforce that the destination of the transport map $\Pi_a$ and $\Pi_p$ which is exactly the joint distribution $Q$ over $(x,a,y)$ we are interested in.

Using the same marignal distribution trick and writing down $d_a((x^A_i, a_i), (x,a)) = d^i_a(x,a)$ and $d_p((x^p_i, y_i), (x,y)) = d^i_p(x,y)$, we can rewrite the primal optimization problem as:
\begin{align*}
    \sup_{Q^a, Q^p} \quad&  \frac{1}{n_p}\sum_{i=1}^{n_p} \int \ell_p(\theta, (x, a, y))  Q^p_i(dx, da, dy)) \\
    \text{s.t.} \quad& \frac{1}{n_a} \sum_{i=1}^{n_a} \int d^i_A(x,a) Q^a_i(dx, da, dy) \le r_a\\
    \quad& \frac{1}{n_p}\sum_{i=1}^{n_p}\int d^p_i(x,y) Q^p_i(dx, da, dy) \le r_p\\
    \quad& \frac{1}{n_a}\sum_{i=1}^{n_a} Q^a_i(x, a, y)) \le \frac{1}{n_p}\sum_{i=1}^{n_p} Q^p_i((x, a, y)) \quad \forall x, a, y\\
    \quad& \frac{1}{n_p}\sum_{i=1}^{n_p} Q^p_i((x^p_i, y_i), (x, a, y)) \le \frac{1}{n_a}\sum_{i=1}^{n_a} Q^a_i(x, a, y) \quad \forall x, a, y\\
    \quad& \int Q^a_i(dx,da,dy) = 1 \quad \forall i \in [n] \\
    \quad& \int Q^p_i(dx,da,dy) = 1 \quad \forall i \in [n] 
\end{align*}
\cj{TODO: be more consistent with the notations i.e. $n^a$}

The corresponding Lagrangian for the above is
\begin{align*}
    &\Lagr(\alpha_A, \alpha_P, \{\beta^a_{x,a,y}\}_{(x,a,y)}, \{\beta^p_{x,a,y}\}_{(x,a,y)}, \{\gamma^{+}_i\}_i, \{\gamma^{-}_i\}_i) \\
    &= \sup_{Q^a, Q^p} 
\end{align*}

\cj{A little worried about the constraints that span over $x,a,y$ right now. I think this won't really be a problem for the joint case because the constraints will simply require that the final $Q^a$ and $Q^p$ are close to the joitn distribution $Q$.} 

Actually, we can instead enforce that the Wasserstein distance should be 0. 
\begin{align*}
    \sup_{Q^a, Q^p, \Pi} \quad&  \frac{1}{n_p}\sum_{i=1}^{n_p} \int \ell_p(\theta, (x, a, y))  Q^p_i(dx, da, dy)) \\
    \text{s.t.} \quad& \frac{1}{n_a} \sum_{i=1}^{n_a} \int d^i_A(x,a) Q^a_i(dx, da, dy) \le r_a\\
    \quad& \frac{1}{n_p}\sum_{i=1}^{n_p}\int d^p_i(x,y) Q^p_i(dx, da, dy) \le r_p\\
    \quad& \int d(z, z') \Pi\left( \frac{1}{n_a}\sum_{i=1}^{n_a}Q^a_i(dz), \frac{1}{n_a}\sum_{i=1}^{n_a} Q^p_i(dz')\right) \le 0 \\
    \quad& \int Q^a_i(dx,da,dy) = 1 \quad \forall i \in [n_a] \\
    \quad& \int Q^p_i(dx,da,dy) = 1 \quad \forall i \in [n_p] 
\end{align*}

Now, writing down the Lagrangian of this problem, we get 
\begin{align*}
    \Lagr(\alpha^a, \alpha^p, \beta, \{\gamma^a_i\}, \{\gamma^p_i\}_i) &= \sup_{Q^a, Q^p, \Pi}  \frac{1}{n_p}\sum_{i=1}^{n_p} \int \ell_p(\theta, (x, a, y))  Q^p_i(dx, da, dy)) \\
    &+ \alpha^a \left(r_a - \frac{1}{n_a} \sum_{i=1}^{n_a} \int d^i_A(x,a) Q^a_i(dx, da, dy) \right)\\
    &+ \alpha^p \left(r_p -  \frac{1}{n_p}\sum_{i=1}^{n_p}\int d^p_i(x,y) Q^p_i(dx, da, dy) \right)\\
    &- \beta \left(\int d(z, z') \Pi\left( \frac{1}{n_a}\sum_{i=1}^{n_a}Q^a_i(dz), \frac{1}{n_a}\sum_{i=1}^{n_a} Q^p_i(dz')\right) \right)\\
    &+ \sum_{i=1}^{n_a} \gamma^a_i \left(1 - \int Q^a_i(dx,da,dy) \right)\\
    &+ \sum_{i=1}^{n_p} \gamma^p_i \left(1 - \int Q^p_i(dx,da,dy) \right)
\end{align*}

Regathering some of the terms for $i \in [n_a]$ and $i \in [n_p]$ separately, we get
\begin{align*}
    \Lagr(\alpha^a, \alpha^p, \beta, \{\gamma^a_i\}, \{\gamma^p_i\}_i) &= \sup_{Q^a, Q^p, \Pi} \frac{1}{n_p}\sum_{i=1}^{n_p}\left(\int \ell_p(\theta, z) - \alpha^p d^p_i(x,y) - n_p\gamma^p_i ) Q^p_i(dz)\right) \\
    &+\frac{1}{n_a}\sum_{i=1}^{n_a}\left(\int - \alpha^a d^i_A(x,y) - n_a\gamma^p_i ) Q^a_i(dz)\right) \\\\
    &- \beta \left(\int d(z, z') \Pi\left( \frac{1}{n_a}\sum_{i=1}^{n_a}Q^a_i(dz), \frac{1}{n_a}\sum_{i=1}^{n_a} Q^p_i(dz')\right) \right)\\
    &+ \sum_{i=1}^{n_a} \gamma^a_i + \sum_{i=1}^{n_p} \gamma^p_i. 
\end{align*}

Not clear how to proceed from here because of the $\beta$ constraint part.. Let me try to be actually more formal and apply Fenchel duality directly which will require calculating the convex conjugates.
\cj{Need to understand Fenchel duality and maybe need to worry about existence of the above problem.}
Then, the constraint becomes
\[
    \sup_{(x,a)} \ell_p(\theta, (x, a, +1)) - \alpha_A ||(x^A_i,a_i) - (x,a)||  -  \alpha_P ||x^P_j - x|| - \frac{\kappa}{2}|y_i-1| - n_P n_A \beta_{i,j} \le 0.
\]

The question now is whether we can use a similar trick to characterize
\[
    \sup_{(x,a)} \ell_p(\theta, (x, a, +1)) - \alpha_A ||(x^A_i,a_i) - (x,a)||  -  \alpha_P ||x^P_j - x||
\]

When we `linearize' things during the conjugation, we may be able collapse/split the $||(x,a) - (x',a')||$ and $||x - x'||$ terms, maybe? 

\begin{lemma}
\begin{align*}
    &\sup_{(x,a)} \ell_p(\theta, (x, a, +1)) - \alpha_A ||(x^A_i,a_i) - (x,a)||  -  \alpha_P ||x^P_j - x|| \\
    &=\begin{cases}
         BLAH\\
         BLAH\\
    \end{cases}
\end{align*}
\end{lemma}
\begin{proof}
We will write $(x, a)$ to denote the concatenation of $x$ and $a$. Then, the loss for each $(x,a,y)$ is 
\[
    h_\beta(x, a) =  \log(1 + \exp(-\langle\beta, (x,a) \rangle)).
\]

If we have $f(t) = \log(1 + \exp(-t))$, then the convex conjugate $f^*$ is 
\begin{align*}
    f^*(\theta) = \begin{cases}
         \theta  \ln \theta  + (1-\theta) \ln(1-\theta) \quad\text{if $\theta \in [0,1]$}\\
         +\infty \quad\text{otherwise}
    \end{cases}
\end{align*}
where $0 \log 0 = 0$. Then, we have $h_\beta(x,a) = f(\langle \beta, (x, a) \rangle)$. 
\begin{align*}
    &\sup_{(x,a)} h_{\beta}((x, a)) - \lambda_1 ||(x^A_i,a_i) - (x,a)||  -  \lambda_2 ||x^P_j - x||\\
    &=\sup_{(x,a)} \sup_{\theta \in [0,1]} \langle\theta\beta, (x,a) \rangle  - f^*(\theta) - \lambda_1 ||(x^A_i,a_i) - (x,a)||  -  \lambda_2 ||x^P_j - x||\\
    &= \sup_{\theta \in [0,1]} \sup_{(x,a)}  \langle\theta\beta, (x,a) \rangle  - f^*(\theta) - \sup_{||q_1||_{*} \le \lambda_1}\langle q_1, (x^A_i,a_i) - (x,a)\rangle -  \sup_{||q_2||_{*} \le \lambda_2}\langle q_2, x^P_j - x\rangle\\
    &= \sup_{\theta \in [0,1]} \sup_{(x,a)} \inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}}  \langle\theta\beta, (x,a) \rangle  - f^*(\theta) - \langle q_1, (x^A_i,a_i) - (x,a)\rangle -  \langle q_2, x^P_j - x\rangle\\
\end{align*}

If $a \in \R^{d}$, we attach a zero vector $0^d \in \R^d$ to $q_2$ and we get 
\begin{align*}
    &= \sup_{\theta\in [0,1]} \sup_{(x,a)} \inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}}  \langle\theta\beta, (x,a) \rangle  - f^*(\theta) - \langle q_1, (x^A_i,a_i) - (x,a)\rangle -  \langle (q_2, 0^d), (x^P_j, 0^d) - (x,a)\rangle\\
    &= \sup_{\theta \in [0,1]} \sup_{(x,a)} \inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}}  \langle\theta\beta +q_1 + (q_2,0^d), (x,a) \rangle  - f^*(\theta) - \langle q_1, (x^A_i,a_i)\rangle -  \langle q_2, x^P_j \rangle
\end{align*}

Note that everything is linear in terms of $\theta, (x,a), q_1,$ and $q_2$ along with convex constraints, so minmax theorem holds here. 
\begin{align*}
    &= \sup_{\theta \in [0,1]} \inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}}  \sup_{(x,a)} \langle\theta\beta +q_1 + (q_2,0^d), (x,a) \rangle  - f^*(\theta) - \langle q_1, (x^A_i,a_i)\rangle -  \langle q_2, x^P_j \rangle
\end{align*}


If $\theta\beta +q_1 + (q_2,0^d) \neq 0$, then we can choose $(x,a)$ to drive the whole thing to $\infty$, so we have
\begin{align*}
    &= \sup_{\theta \in [0,1]} \inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}} \begin{cases} \infty &\quad\text{ if $\theta\beta +q_1 + (q_2,0^d) \neq 0$}\\
    - f^*(\theta) - \langle q_1, (x^A_i,a_i)\rangle -  \langle q_2, x^P_j \rangle &\quad\text{otherwise}
    \end{cases}
\end{align*}

If there doesn't exist $(q_1,q_2)$ such that they add up to $-\beta$, then the $\sup$ can choose $\theta=1$ so that everything evaluates to $\infty$. \cj{Actualy, this dimensionality issue is making things a little confusing..} Therefore, suppose not. Then, note that the latter terms can be shown to be an infimal convolution. More specifically, write 
\begin{align*}
    g^i_1(q) = \begin{cases}
         -\langle q, (x^A_i, a_i) \rangle \quad\text{if $||y||_{*} \le \lambda_1$}\\
         \infty
    \end{cases}
    \quad\text{and}\quad
    g^j_2(q) = \begin{cases}
         -\langle q, (x^P_j, 0^d) \rangle \quad\text{if $||y[1:n]||_{*} \le \lambda_2$}\\
         \infty
    \end{cases}    
\end{align*}

Then, we see that the latter terms is an infimal convolution of $g^i_1$ and $g^j_2$:
\begin{align*}
    &= \sup_{\theta \in [0,1]} -f^*(\theta) + (g^i_1 \square g^j_2)(\theta\beta),
\end{align*}
where $(g^i_1 \square g^j_2)(q) = \inf_{q_1 + q_2 = q} g^i_1(q_1 + g^i_1(q_2)$ is the infimal convolution of $g^i_1$ and $g^j_2$.

\begin{lemma}
Suppose $g^i_1(q) = \langle q, x_1 \rangle$ if $q \in B_1$ and $\infty$ otherwise, and $g^j_2(q) = \langle q, x_2 \rangle$ if $q \in B_2$ and $\infty$ otherwise. 
    \begin{align*}
        (g^i_1 \square g^j_2)(q) \le \min(\langle q, x_1\rangle, \langle q, x_2 \rangle)
    \end{align*}
\end{lemma}
\begin{proof}
    \begin{align*}
        (g^i_1 \square g^j_2)(q) \le \min(\langle q, x_1\rangle + \langle 0, x_2 \rangle, \langle 0, x_1\rangle + \langle q, x_2 \rangle \rangle) \le \min(\langle q, x_1\rangle, \langle q, x_2 \rangle)
    \end{align*}
\end{proof}

\begin{lemma}
Suppose $g^i_1(q) = \langle q, x_1 \rangle$ if $q \in B_1$ and $\infty$ otherwise, and $g^j_2(q) = \langle q, x_2 \rangle$ if $q \in B_2$ and $\infty$ otherwise.
Given $q$ such that there exists some $q_1 \in B_1$ and $q_2 \in B_2$ such that $q_1 + q_2 = q$, then we have
\[
    (g^i_1 \square g^j_2)(q) \ge \min(\langle q, x_1 \rangle, \langle q, x_2 \rangle)
\]
\end{lemma}
\begin{proof}
Note that for any $q_1 \in B_1$ and $q_2 \in B_2$,
\begin{align*}
    \min(g^i_1(q_1), g^j_2(q_1)) + \min(g^i_1(q_2), g^j_2(q_2)) \ge \min(\langle q_1 + q_2, x_1 \rangle, \langle q_1 + q_2, x_2 \rangle) 
\end{align*}
When does this hold true??
\begin{align*}
    \inf_{q_1 + q_2 = q} \min(g^i_1(q_1), g^j_2(q_1)) + \min(g^i_1(q_2), g^j_2(q_2))
    \ge \min(\langle q, x_1 \rangle, \langle q, x_2 \rangle).
\end{align*}
Therefore, we have
\begin{align*}
    (g^i_1 \square g^j_2)(q) &= \inf_{q_1 + q_2 = q} g^i_1(q_1) + g^j_2(q_2)\\
    &\ge \inf_{q_1 + q_2 = q} \min(g^i_1(q_1), g^j_2(q_1)) + \min(g^i_1(q_2), g^j_2(q_2))\\
    &\ge \min(\langle q, x_1 \rangle, \langle q, x_2 \rangle).
\end{align*}

$(g^i_1 \wedge g^j_2)(q_1) + (g^i_1 \wedge g^j_2)(q_2)$\\
$\ge(g^i_1 \wedge g^j_2)(q_1 + q_2) = \min(g^i_1(q), g^j_2(q))$

\end{proof}



\cj{I thought that the conjugates will add up nicely but they actually don't add up too nicely because of the norm constraint. I wonder if trying to get a handle on this through geometry (previous route) is still the way to go. Also, maybe, instead of trying to get a closed form for this, maybe noting that everything is easy to evaluate (convex optimization problem) and we can calculate the gradient pretty easily is enough (as for the gradient, I'm actually not sure how easy this is.)}
\cj{The subadditive method looks promising! }
\cj{Big assumption!}
Suppose we are interested in $y$ (which will be our $\theta\beta$) such that $||y||_{*} \le \lambda_1$ and $||y[1:n]||\le \lambda_2$ are equivalent: no matter what $y[n+1:n+d]$ is, we have $||y||_{*} \le \lambda_1$ implies $||y[1:n]||\le \lambda_2$ and $||y[1:n]||\le \lambda_2$ implies $||y||_{*} \le \lambda_1$. 

Then, we have $g^i_1(y - )$



Then, we can write
\begin{align*}
    &= \sup_{\theta \in [0,1]} - f^*(\theta) + \left(g^i_1 \square g^j_2 \right)(\theta\beta)
\end{align*}
where $(g^i_1 \square g^j_2)(y) = \inf_{q_1 + q_2 = y}(g^i_1(q_2) + g^j_2(q_2))$ is the infimal convolution of $g^i_1$ and $g^j_2$.

One useful fact about the infimal convolution is that its convex conjugate is the sum of the underlying function's convex conjugate.
\[
    (g^i_1 \square g^j_2)^*(y^*) = g^*_1(y^*) + g^*_2(y^*).
\]
Note that 
\begin{align*}
    g^*_1(y^*) &= \sup_{y} \langle y, y^* \rangle - g^i_1(y)\\
    &= \sup_{y: ||y||_{*} \le \lambda_1} \langle y, y^* \rangle + \langle y, (x^A_i, a_i) \rangle\\
    &= \sup_{y: ||y||_{*} \le \lambda_1} \langle y, y^* + (x^A_i, a_i) \rangle\\
    &= \lambda_1||y^* + (x^A_i, a_i)||
\end{align*}
\cj{forget about the funky dimensionality issue for now: if we can't get around it, we can do the same thing as $y$ and just blow up the number of constraints by the possible $a$ values.}
\begin{align*}
    g^*_2(y^*) &= \sup_{q} \langle q, y^* \rangle - g^j_2(q)\\
    &= \sup_{q} \begin{cases}
         \langle  q, (y^* + (x^P_j, 0^d))\rangle \quad\text{if $||q[1:n]||_{*} \le \lambda_2$}\\
         -\infty
    \end{cases}\\
    &= \lambda_1 ||y^*+(x^P_j, 0^d)||.
\end{align*}

Note that $g^*_2(y^*) = g^*_1(y^* - (x^p_{i}, a_i))$






We have
\begin{align*}
    (g^i_1 \square g^j_2)^{**}(y) &= \sup_{y^*} \langle y^*, y \rangle - (g^i_1 \square g^j_2)^*(y^*) \\
    &= \sup_{y^*} \langle y^*, y \rangle - (g^i_1 \square g^j_2)^*(y^*) \\
    &= \sup_{y^*} \langle y^*, y \rangle -  \left(|| y^* + (x^A_i, a_i)|| + \sup_{q} \begin{cases}
         \langle  q, y^* + (x^p_i, a_i)\rangle \quad\text{if $||q[1:n]||_{*} \le \lambda_2$}\\
         -\infty
    \end{cases}\right) 
\end{align*}

Therefore, we have \cj{Working on this...}
\begin{align*}
    (g^i_1 \square g^j_2)(y) = \begin{cases}
         BLAH \\
         \infty \quad\text{otherwise}
    \end{cases}
\end{align*}


For simplicity, we'll just focus on the case where $\lambda_1 \le \lambda_2$.

Then, we get
\begin{align*}
    &= \sup_{\theta \in [0,1]} -f^*(\theta) + \theta \left((g^i_1 \square g^j_2)(\beta)\right)\\
    &=f((g^i_1 \square g^j_2)(\beta)).
\end{align*}



\cj{TODO: Keep some stuff that demonstrates what's happening at a high level -- it's loss minus the distance between $x^A_i$ and $x^j_p$.}
\begin{enumerate}
    \item $||\beta||_{*} + \lambda_2 \le \lambda_1$.\\
Substituting $(q_2, 0^d)$ with $\beta\theta - q_1$, we have
\begin{align*}
    &=\sup_{\theta \in [0,1]}\inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}} \begin{cases} \infty &\quad\text{ if $\theta\beta +q_1 + (q_2,0^d) \neq 0$}\\ - f^*(\theta) - \langle -\theta\beta-(q_2,0^d), (x^A_i,a_i)\rangle -  \langle (q_2, 0^d), (x^P_j,a_i)\rangle &\quad\text{otherwise}
    \end{cases}\\
    &=\sup_{\theta \in [0,1]} \inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}} \begin{cases} \infty &\quad\text{ if $\theta\beta +q_1 + (q_2,0^d) \neq 0$}\\
     - f^*(\theta) + \langle \theta\beta, (x^A_i,a_i)\rangle -  \langle (q_2, 0^d), (x^P_j,a_i) - (x^A_i, a_i) \rangle &\quad\text{otherwise}
     \end{cases}\\
    &=\sup_{\theta \in [0,1]} \inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}} \begin{cases} \infty &\quad\text{ if $\theta\beta +q_1 + (q_2,0^d) \neq 0$}\\
     - f^*(\theta) + \langle \theta\beta, (x^A_i,a_i)\rangle -  \langle q_2, x^P_j - x^A_i \rangle &\quad\text{otherwise}
    \end{cases}\\
\end{align*}
    For the feasible space, for $q_2$, we'll write
\[
N(\theta\beta, \lambda_1, \lambda_2) = \{q_2: ||q_2||_{*} \le \lambda_2, \exists q_1: ||q_1||_{*} \le \lambda_1, \theta\beta + q_1 + (q_2,0^d) = 0\}.
\]
Then, we have
\begin{align*}
    &\sup_{\theta \in [0,1]} \left(- f^*(\theta) + \langle \theta\beta, (x^A_i,a_i)\rangle + \inf_{q_2 \in N(\theta\beta, \lambda_1, \lambda_2)}- \langle q_2, x^P_j - x^A_i \rangle\right)\\
\end{align*}

However, in this case where $||\beta||_{*} + \lambda_2 \le \lambda_1$, we have $N(\beta\theta, \lambda_1, \lambda_2) = \{q_2: ||q_2||_{*} \le \lambda_2\}$ no matter which $\theta$ is chosen. 
Then, we have
\begin{align*}
    &=h_{\beta}((x^A_i,a_i)) +  \inf_{||q_2||_{*} \le \lambda_2} - \langle (q_2, 0^d), x^P_j - x^A_i \rangle \\
    &=h_{\beta}((x^A_i,a_i)) +  \inf_{||q_2||_{*} \le \lambda_2} \langle q_2,  x^A_i - x^P_j \rangle \\
    &=h_{\beta}((x^A_i,a_i)) -  \sup_{||q_2||_{*} \le \lambda_2} \langle q_2,  x^P_j - x^A_i  \rangle \\
    &=h_{\beta}((x^A_i,a_i)) -  \lambda_2 ||x^P_j  - x^A_i ||. 
\end{align*}
    \item $||\beta||_{*} + \lambda_1 \le \lambda_2.$\\
Similar technique can be used here. 
Substituting $q_1$ with $\beta\theta - (q_2, 0^d)$, we have
\begin{align*}
    &=\sup_{\theta \in [0,1]}\inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}} \begin{cases} \infty &\quad\text{ if $\theta\beta + q_1 + (q_2,0^d) \neq 0$}\\ - f^*(\theta) - \langle q_1, (x^A_i,a_i)\rangle -\langle -\theta\beta-q_1, (x^P_j,a_i)\rangle  &\quad\text{otherwise}
    \end{cases}\\
    &=\sup_{\theta \in [0,1]} \inf_{\substack{||q_1||_{*} \le \lambda_1,\\ ||q_2||_{*} \le \lambda_2}} \begin{cases} \infty &\quad\text{ if $\theta\beta +q_1 + (q_2,0^d) \neq 0$}\\
     - f^*(\theta) + \langle \theta\beta, (x^P_j,a_i) \rangle - \langle q_1, (x^A_i, a_i)-(x^P_j,a_i) \rangle &\quad\text{otherwise}
     \end{cases}\\
\end{align*}
    For the feasible space, for $q_1$, we'll write
\[
N(\theta\beta, \lambda_1, \lambda_2) = \{q_1: ||q_1||_{*} \le \lambda_1, \exists q_2: ||q_2||_{*} \le \lambda_2, \theta\beta + q_1 + (q_2,0^d) = 0\}.
\]
\cj{TODO: distinguish between the $N$ in the first case and this. And instead of $N$, might be better to use another symbol just because $N$ sounds like the number of data points.}
Then, we have
\begin{align*}
    &\sup_{\theta \in [0,1]} \left(- f^*(\theta) + \langle \theta\beta, (x^A_i,a_i)\rangle + \inf_{q_2 \in N(\theta\beta, \lambda_1, \lambda_2)}- \langle q_1, (x^A_i, a_i)-(x^P_j,a_i) \rangle\right)\\
\end{align*}

However, in this case where $||\beta||_{*} + \lambda_1 \le \lambda_2$, we have $N(\beta\theta, \lambda_1, \lambda_2) = \{q_2: ||q_2||_{*} \le \lambda_2\}$ no matter which $\theta$ is chosen. 
Then, we have
\begin{align*}
    &=h_{\beta}((x^P_j,a_i)) +  \inf_{||q_1||_{*} \le \lambda_1} - \langle q_1, (x^A_i, a_i)-(x^P_j,a_i) \rangle \\
    &=h_{\beta}((x^A_i,a_i)) -  \sup_{||q_1||_{*} \le \lambda_1} \langle q_1,  (x^A_i, a_i)-(x^P_j,a_i) \\
    &=h_{\beta}((x^A_i,a_i)) -  \lambda_1 || (x^A_i, a_i)-(x^P_j,a_i) ||. 
\end{align*}
    
    \item $||\beta||_{*} > |\lambda_1 - \lambda_2|.$\\
This is the tricky part because both terms still depend on $\theta$.
Since $\lambda_1$ and $\lambda_2$'s are both inputs that the user can specify as parameters to the original primal optimization problem (i.e. they correspond to the radius of the Wasserstein balls), we'll simply assume $\lambda_2 \ge \lambda_1$ and go with the substitution of the first case. 
\begin{align*}
    &\sup_{\theta \in [0,1]} \left(- f^*(\theta) + \theta \langle \beta, (x^A_i,a_i)\rangle + \inf_{q_2 \in N(\theta\beta, \lambda_1, \lambda_2)}- \langle q_2, x^P_j - x^A_i \rangle\right)\\
    &=\sup_{\theta \in [0,1]} \left(- f^*(\theta) + \theta \langle \beta, (x^A_i,a_i)\rangle - \sup_{q_2 \in N(\theta\beta, \lambda_1, \lambda_2)} \langle q_2, x^A_i - x^P_j \rangle\right)\\
\end{align*}



\cj{Have a much better idea of how $N$ behaves. The closed form involves a arcos (inverse of cosine), but I think calculating the value will be easy. Also, I think the second term is concave in $\theta$. So, I think finding the $\sup_{\theta \in [0,1]}$ should be feasible. It's just not clear whether there'll be a clean closed form solution.}\cj{It'll help to have some drawing.. I'll try to take a screenshot and upload it here..}

\cj{Ignoring dimensionality issue}
\[
N(\theta\beta, \lambda_1, \lambda_2) = \{q_1: ||q_1||_{*} \le \lambda_1, \exists q_2: ||q_2||_{*} \le \lambda_2, \theta\beta + q_1 + (q_2,0^d) = 0\}.
\]
Consider two spheres whose norms are bounded by $\lambda_1$ and $\lambda_2$ respectively, but the second sphere's center is shifted by $-\theta\beta$:
\[
    S_1 = \{q_1: || q_1 || \le \lambda_1  \}
\]
and
\[
    S_2 = \{q_2: || q_2 + \theta\beta || \le \lambda_2 \}.
\]

\begin{lemma}
    $N$ can be describe as a spherical sector that is formed as a result of the intersection of $S_1$ and $S_2$:
    \[
        N(\theta\beta, \lambda_1, \lambda_2) = \{q:  q \in S_1 \cap S_2 \}.
    \]
\end{lemma}
\begin{proof}
First, it's easy to see that 
\[
    \{q:  q \in S_1 \cap S_2 \} \subseteq N(\theta\beta, \lambda_1, \lambda_2).
\]
For any $q_1 \in S_1 \cap S_2$, take $q_2 = -\theta\beta-q_1$. By construction, $q_1 + q_2 = -\theta\beta$, and because $q_1 \in S_1 \cap S_2$, we have that the distance from $q_1$ to the center of the second sphere is at most $\lambda_2$: $||-\beta\theta - q_1 || \le \lambda_2$, meaning $||q_2|| \le \lambda_2$. 

Now, we try to prove the other case -- that is
\[
     N(\theta\beta, \lambda_1, \lambda_2) \subseteq \{q:  q \in S_1 \cap S_2 \}. 
\]
Take any $q_1 \in N(\theta\beta, \lambda_1, \lambda_2)$ and its corresponding $q_2$ such that $||q_2|| \le \lambda_2$ and $q_1 + q_2 = -\theta\beta$. Now, for the sake of contradiction, assume $q_1 \not\in S_1 \cap S_2$. Because $||q_1|| \le \lambda_1$, this means $q_1 \not\in S_2$, meaning its distance to $\theta\beta$ will be more than $\lambda_2$: that is, $||-\theta\beta - q_1|| > \lambda_2$. However, that means $||q_2|| > \lambda_2$, which is a contradiction.
\end{proof}
\cj{It shows that the feasible region $N(\theta\beta, \lambda_1, \lambda_2)$ is a convex region.. So, it's a linear optimization with a convex set. }


\cj{Linear optimization with convex set means the solution is at the boundary of the set -- meaning $||q_1|| = \lambda_1$ or $||q_2||=\lambda_2$ -- I feel like we should be able to tell which case we should be in depending on $\lambda_1 > \lambda_2$ or not.}
\cj{Suppose we have that $||q_1|| = \lambda_1$. Then, among all $q_1 \in S_1 \cap S_2$ such that $||q_1|| = \lambda_1$, which $q_1$ should maximize the the inner product with $x$? The one with the smallest angle with $x$. That means we must have that $||q_1||=\lambda_1$ and $||q_2|| = \lambda_2$! This last part needs more elaboration. Actually, this might not be true?}
\cj{What if $\lambda_1 = \lambda_2$? Then by symmetry, should we have that they should be both tight?}\cj{Tried out some experiments to see how they behave, but I don't think things will be concave in $\theta$. }
\cj{Trying to think of when we can kind of approximate things. For instance what if we only match pairs where $||x-x'||$ is sufficiently small. Then, just approximating it with the above two cases may be fine?}


\cj{There is more literature on this thing called Moreau-Yosida regularization, which is a special case of infimal convolution. Trying to understand the concept a bit better to see if it applies to our setting}
\begin{lemma}
\cj{In Progress: angle lemma}
If $\frac{\lambda_1}{||x||} x \not\in N(\theta\beta, \lambda_1, \lambda_2)$, then
\[
\sup_{q_1 \in N(\theta\beta, \lambda_1, \lambda_2)} \langle q_1, x \rangle = ||q_1|| \cdot ||x|| \cdot \cos(a) \]
where the angle is $a = \frac{\langle x, \theta\beta \rangle}{|| x|| \cdot || \theta\beta||} - \arccos\left(\frac{\lambda_1^2 +||\theta\beta||^2 - \lambda_2^2}{2 || \theta\beta|| \lambda_1 }\right)$.
\end{lemma}
\begin{proof}
\[
    \arg\max_{q_1 \in N(\theta\beta, \lambda_1, \lambda_2)} \langle q_1, x \rangle = BLAH
\]
First, we show that $q_1$ that achieves the sup must be on the boundary of $N(\theta\beta, \lambda_1, \lambda_2)$. 



Then, we can consider the triangle formed by the origin, $q_1$, and $\beta\theta$. Using the law of cosines, we get .



Then, we can use the law of cosines to show that the angle between the boundary and the $x$  will be as stated in the lemma.

\cj{Hmm actually, the picture was deceiving....}
\end{proof}


\begin{lemma}
\[
    \cos(a + \arccos(b)) = BLAH
\]
\end{lemma}
\begin{proof}
    Not sure what trig equalities Wolfram Alpha is leveraging, but need to figure that out first.
\end{proof}

\end{enumerate}

\cj{Some thought. When transporting. We can decide to transport between $i$ and $j$th example if and only if $x$'s are actually close so as to avoid considering $n^2$ pairs.}



\cj{SCRATCH EVERYTHING ABOVE!}
Instead of substituting in via the equality $\theta\beta + q_1 + q_2 =0$, and only looking at one of them separately, we should look at them together because they together form an infimal convolution. 

Given two proper functions $f$ and $g$, infimal convolution is written as \[
    (f \square g)(x) = \inf_{x_1 + x_2 = x} \left( f(x_1) + g(x_2) \right). 
\]

\cj{Two possible routes that I foresee us using}
One useful fact about infimal convolution of two proper functions is 
\[
(f \square g)^*(x) = f^*(x) + g^*(x).
\]

Another useful characterization of the infimal convolution is via their epigraphs where 
\[
    (f \square g)(x) = \inf\{r \in \mathbb{R} | (x,r) \in \epi f + \epi g\}
\]
where $\epi f = \{(x,r) | f(x) \le r\}$ and the sum of two sets is the Minkowski sum.




\iffalse
\cj{OLD STUFF BELOW}
\begin{align*}
    \alpha_A || (x^a,a) - (x',a')|| &= \sup_{||\lambda_1||_{*} \le \alpha} \langle\lambda_1, (x^a,a) - (x',a') \rangle = \sup_{||\lambda_1||_{*} \le \alpha} \langle \lambda_1[1:d], x^a-x'\rangle + \langle \lambda_1[d+1:], a-a'\rangle \\
    \alpha_P || x^p - x'|| &= \sup_{||\lambda_2||_{*} \le \alpha} \langle\lambda_2, x^p - x' \rangle \\
\end{align*}

\cj{Conjecture below: If you jump to the end of the proof in the other paper (assuming everything in this case goes through up until that point as well) and using their notation, you get}
\begin{align*}
    &\sup_{0 \le \theta \le 1} \inf_{\substack{||q_1||_{*}\le \lambda_1,\\ ||q_2||_{*}\le \lambda_2}} \sup_{(x,a)} \langle\theta \beta, (x,a) \rangle - f^*(\theta) - \langle q_1 , (x^A_i, a_i) - (x,a) \rangle - \langle q_2 , x^p_i - x \rangle \\
    &= \sup_{0 \le \theta \le 1} \inf_{\substack{||q_1||_{*}\le \lambda_1,\\ ||q_2||_{*}\le \lambda_2}} \sup_{(x,a)} \langle \theta \beta + q_1 + q'_2, (x,a) \rangle - f^*(\theta) - \langle q_1 , (x^A_i, a_i) \rangle - \langle q_2 , x^p_i \rangle \\
\end{align*}

$x^i \in R^d$
$a^i \in R^l$
$q_1 \in R^{d+l}$

$q_2 \in R^d$

$q'_2 \in R^{d+l}$
$q'_2 = q_2, 0, 0, 0 ,0 ,0 , 0 $
\[
    \langle q'_2, x^{p'}_i - x' \rangle
\]


Can use the first order condition to find that $(x,a)$ should be. However, is it possible to transform $f^*$ back into $f$ and ultimately $h$ term?

Hmmm not clear actually...


Actually, I think we may be able to combine the last inner product terms and combine into one, so that it's like one inner product. 
\begin{align*}
    &= \sup_{0 \le \theta \le 1} \inf_{\substack{||q_1||_{*}\le \lambda_1,\\ ||q_2||_{*}\le \lambda_2}} \sup_{(x,a)} \langle \theta \beta + q_1 + q'_2, (x,a) \rangle - f^*(\theta) - \langle q_1  + q'_2 , (x^A_i, a_i) + (x^p_i, 0) \rangle + \langle q_1, (x^p_i, 0) \rangle + \langle q'_2, (x^A_i, a_i) \rangle
\end{align*}

\begin{align*}
    &= \sup_{0 \le \theta \le 1} \inf_{\substack{||q_1||_{*}\le \lambda_1,\\ ||q_2||_{*}\le \lambda_2}}\begin{cases} - f^*(\theta) - \langle q_1  + q'_2 , (x^A_i, a_i) + (x^p_i, 0) \rangle - \langle q_1, (x^A_i, a_i) \rangle - \langle q'_2, (x^P_j, 0) \rangle \\
    \infty \quad \text{if $\theta \beta + q_1 + q_2 \neq 0$}
    \end{cases}\\
    &= \sup_{0 \le \theta \le 1}\inf_{\substack{||q_1||_{*}\le \lambda_1,\\ ||q_2||_{*}\le \lambda_2}}\begin{cases}  - f^*(\theta) + \langle \theta \beta, (x^A_i, a_i) + (x^p_i, 0) \rangle  - \langle q_1, (x^p_i, 0) \rangle - \langle q'_2, (x^A_i, a_i) \rangle \\
    \infty \quad \text{if $\theta \beta + q_1 + q_2 \neq 0$}
    \end{cases}\\
    &= \sup_{0 \le \theta \le 1}\inf_{||q_1||_{*}\le \lambda_1}\begin{cases}  - f^*(\theta) + \langle \theta \beta, (x^A_i, a_i) + (x^p_i, 0) \rangle  - \langle q_1, (x^p_i, 0) \rangle - \langle \theta\beta - q_1, (x^A_i, a_i) \rangle \\
    \infty \quad \text{if $\theta \beta + q_1 + q_2 \neq 0$}
    \end{cases}\
    &= \sup_{0 \le \theta \le 1}\inf_{||q_1||_{*}\le \lambda_1}\begin{cases}  - f^*(\theta) + \langle \theta \beta, (x^A_i, a_i) + (x^p_i, 0) \rangle  - \langle q_1, (x^p_i, 0) \rangle - \langle \theta\beta - q_1, (x^A_i, a_i) \rangle \\
    \infty \quad \text{if $\theta \beta + q_1 + q_2 \neq 0$}
    \end{cases}
\end{align*}

Actually the inf term can be formulated as a linear minimization problem with dual norm constraints.
\cj{somewhat solved it. transcribing over here}
\begin{align*}
    &= \sup_{0 \le \theta \le 1} \inf_{\substack{||q_1||_{*}\le \lambda_1,\\ ||q_2||_{*}\le \lambda_2}}\begin{cases} - f^*(\theta) - \langle q_1 , (x^A_i, a_i) \rangle - \langle q_2 , x^P_j \rangle \\
    \infty \quad \text{if $\theta \beta + q_1 + q_2 \neq 0$}
    \end{cases}\\
    &= \sup_{0 \le \theta \le 1} \inf_{\substack{||q_2||_{*}\le \lambda_2,\\ ||\theta\beta - q_2 ||_{*} \le \lambda_1}} \begin{cases}- f^*(\theta) +\langle \theta \beta, (x^A_i, a_i)\rangle + \langle q_2, (x^A_i,a_i) - x^P_j \rangle \quad\text{if $||\theta \beta||_{*} \le \lambda_1 + \lambda_2$} \\ \infty \end{cases}\\
    &= \sup_{0 \le \theta \le 1} - f^*(\theta) +\langle \theta \beta, (x^A_i, a_i) \rangle +  \inf_{\substack{||q_2||_{*}\le \lambda_2,\\ ||\theta\beta - q_2 ||_{*} \le \lambda_1}}  \begin{cases}\langle q_2, (x^A_i,a_i) - x^P_j \rangle \quad\text{if $||\beta||_{*} \le \lambda_1 + \lambda_2$}\\ \infty \end{cases}\\
\end{align*}

If $||\beta||_{*} \le \lambda_1 + \lambda_2$, then we have
\begin{align*}
    \sup_{0 \le \theta \le 1} - f^*(\theta) +\langle \theta \beta, (x^A_i, a_i) \rangle +  \inf_{\substack{||q_2||_{*}\le \lambda_2,\\ ||\theta\beta - q_2 ||_{*} \le \lambda_1}}  \langle q_2, (x^A_i,a_i) - x^P_j \rangle\\
\end{align*}

Below is what needs to be kind of ironed out.
If $||\theta\beta - q_2|| \le \lambda_1$ is not binding and we can drop it, then we get
\begin{align*}
    &= \sup_{0 \le \theta \le 1} - f^*(\theta) +\langle \theta \beta, (x^A_i, a_i) \rangle +  \inf_{||q_2||_{*}\le \lambda_2}  \langle q_2, (x^A_i,a_i) - x^P_j \rangle \\
    &= h_\beta((x^A_i, a_i)) + \lambda_2 || (x^A_i, a_i) - x^P_j||  \\
\end{align*}

I wonder it will be binding in the only one case, so we just get
\[
    h_\beta((x^A_i, a_i)) + \lambda_2 || (x^A_i, a_i) - x^P_j|| 
\]
and
\[
    h_\beta((x^p_i, 0)) + \lambda_1 || (x^A_i, a_i) - x^P_j|| 
\]
In general, I don't think that can be just dropped actually.... For instance if $\theta \beta$ is pointing toward the opposite direction as $(x^A_i,a_i - x^P_j)$, then the term might be actually be negative.
Actually, if $\theta=1$, unless these two vectors are pointing toward the same direction, they are not going to be the same value as the norm (the value where the constraint is dropped).
\fi

\end{proof}




\iffalse
\begin{align}
\begin{split}
    \sup_{\{Q_{i,j}\}_{i,j}} \quad&  \frac{1}{n_p n_a}\sum_{i=1}^{n_a}\sum_{j=1}^{n_p} \int \ell_p(\beta, (x, a, +1))  Q^{+1}_{i,j}(dx, da)) + \int \ell_p(\beta, (x, a, -1))  Q^{-1}_{i,j}(dx, da) \\
    \text{s.t.} \quad& \frac{1}{n_p n_a}\sum_{i=1}^{n_a}\sum_{j=1}^{n_p} \int d^i_A(x,a)  Q^{+1}_{i,j}(dx, da) + \int d^i_A(x,a)  Q^{-1}_{i,j}(dx, da) \le r_a\\
    \quad& \frac{1}{n_p n_a} \sum_{j=1}^{n_p} \sum_{i=1}^{n_a} \int d^j_P(x,y)  Q^{+1}_{i,j}(dx, da) + \int d^j_P(x,y)  Q^{-1}_{i,j}(dx, da) \le r_p\\
    \quad& \int Q^{+1}_{i,j}(dx,da) + Q^{-1}_{i,j}(dx,da) = 1 \quad \forall i \in [n_a], j \in [n_p] \\
\end{split}
\label{eqn:primal-disjoint1}
\end{align}

\cj{Moving $a$ into $Q$ like we did for $y$ just to avoid dimensionality issue in the dual. We can think about how to avoid this, once we solve everything without the dimensionality issue.}
Let $A=\{a_1, \dots, \}$ denote all possible. values that $a$ can take.
\begin{align}
\begin{split}
    \sup_{\{Q_{i,j}\}_{i,j}} \quad&  \frac{1}{n_p n_a}\sum_{i=1}^{n_a}\sum_{j=1}^{n_p} \sum_{a \in A}\int \ell_p(\theta, (x, a, +1))  Q^{+1, a}_{i,j}(dx) + \int \ell_p(\theta, (x, a, -1))  Q^{-1, a}_{i,j}(dx) \\
    \text{s.t.} \quad& \frac{1}{n_p n_a}\sum_{i=1}^{n_a}\sum_{j=1}^{n_p} \sum_{a \in A}\int d^i_A(x,a)  Q^{+1, a}_{i,j}(dx) + \int d^i_A(x,a)  Q^{-1, a}_{i,j}(dx) \le r_a\\
    \quad& \frac{1}{n_p n_a} \sum_{j=1}^{n_p} \sum_{i=1}^{n_a} \sum_{a \in A}\int d^j_P(x,y)  Q^{+1, a}_{i,j}(dx) + \int d^j_P(x,y)  Q^{-1, a}_{i,j}(dx) \le r_p\\
    \quad& \int \left(\sum_{a \in A} Q^{+1, a}_{i,j}(dx) + \sum_{a \in A} Q^{-1, a}_{i,j}(dx) \right)= 1 \quad \forall i \in [n_a], j \in [n_p] \\
\end{split}
\label{eqn:primal-disjoint2}
\end{align}
\fi

\iffalse
In fact, the same proof works to show that strong duality holds between the primal problem \eqref{eqn:primal-disjoint1} and the following dual problem:
\begin{align}
\begin{split}
    \inf_{\alpha_A, \alpha_P, \{\beta_{i,j}\}_{i,j}} \quad& \alpha_A r_a + \alpha_P r_p + \sum_{i\in [n_a], j\in[n_p]} \beta_{i,j}\\
    \text{such that} \quad& \sup_{(x,a)} \ell_p(\theta, (x, a, +1)) - \alpha_A d^i_A(x,a)  -  \alpha_P d^j_P(x,+1) - n_p n_a \beta_{i,j} \le 0 \quad i \in [n_a], j \in [n_p]\\
    & \sup_{(x,a)} \ell_p(\theta, (x, a, -1)) - \alpha_A d^i_A(x,a)  -  \alpha_P d^j_P(x,-1) - n_p n_a \beta_{i,j} \le 0 \quad i \in [n_a], j \in [n_p]
\end{split}
\label{eqn:dual-disjoint-dual1}
\end{align}
\fi

First, note that the optimization problem \eqref{eqn:optimization1} is jointly convex in $(\alpha_A, \alpha_P)$ and $\theta$. So, fixing $(\theta, \alpha_A)$, the objective function is convex in $\alpha_P$, and similarly, fixing $(\theta, \alpha_P)$, the objective function is convex in $\alpha_A$. In other words, if we know that $\alpha_A^* \in [0, u_A]$ $\alpha_P^* \in [0, u_P]$ and we can solve the optimization problem for fixed $(\alpha_A, \alpha_P)$, then we can use golden-section search alternatively over $[0, u_A]$ and $[0, u_P]$ in order to find $\alpha^*_A$ and $\alpha^*_P$. Here's a pseudocode for the golden-section search algorithm:


\begin{algorithm}[H]
    \caption{$\mathtt{GoldenSection}(f, u, \epsilon)$}
    \label{alg:goldenSection}
    \begin{algorithmic}
        \STATE $g = \frac{\sqrt{5} + 1}{2}$
        \STATE $a=0$
        \STATE $b=u$
        \STATE $c = b - (b - a) / g$
        \STATE $d = a + (b - a) / g$
        \WHILE{$|b - a| > \epsilon$}
            \IF{$f(c) < f(d)$}
                \STATE $b = d$
            \ELSE
                \STATE $a=c$
            \ENDIF
            \STATE $c = b - (b - a) / g$
            \STATE $d = a + (b - a) / g$
        \ENDWHILE
        \STATE Output $\frac{a+b}{2}$.
    \end{algorithmic}
\end{algorithm}
\begin{claim}
    Total number of $f$ evaluations in $\mathtt{GoldenSection}(f, u, \epsilon)$ is $O(\log(\frac{u}{\epsilon}))$.
\end{claim}

And suppose we can solve the optimization problem for some fixed $\alpha_A$ and $\alpha_P$ via 
\[
    \mathtt{DROJoinFixedAlphas}(\alpha_A, \alpha_P) = \theta^*_{\alpha_A, \alpha_P} = \arg\min_{\theta} \Omega(\theta, \alpha_A, \alpha_P).
\]

Then, for fixed $\alpha_A$, we may use $\mathtt{DROJoinFixedAlphas}(\alpha_A, \alpha_P)$ as a subroutine to perform golden-section search to find the optimal $\alpha_P$: 
\begin{align*}
    \mathtt{GoldenSectionA}(\alpha_A) &= \mathtt{GoldenSection}(\alpha_P \mapsto \Omega(\alpha_A, \alpha_P, \theta^*_{\alpha_A, \alpha_P}), u_P, \epsilon)\\
    &\approx \arg\min_{\alpha_P} \Omega(\theta^*_{\alpha_A, \alpha_P}, \alpha_A, \alpha_P).
\end{align*}
Then, we can use $\mathtt{GoldenSectionA}(\alpha_A)$ as a subroutine to golden-section search to find the optimal $\alpha_A$:
\begin{align*}
    \mathtt{DROJoin}(\epsilon) &= \mathtt{GoldenSection}(\alpha_A \mapsto \Omega(\alpha_A, \mathtt{GoldenSectionA}(\alpha_A), \theta^*_{\alpha_A, \alpha_P}), u_A, \epsilon).
\end{align*}

Note that there will be a total of $O(\log(u_A))$ many oracle calls to $\mathtt{DROJoinFixedAlphas}$ in $\mathtt{GoldenSectionA}$, and similarly, $O(\log(u_P))$ many oracle calls to $\mathtt{GoldenSectionA}$ for $\mathtt{DROJoin}$. Therefore, there will be a total of $O(\log^2(\max{(u_A, u_P)})$ many oracle calls to $\mathtt{DROJoinFixedAlphas}$ in $\mathtt{DROJoin}(\epsilon)$.



Now, we describe how we can find $u_A$ and $u_P$ via some doubling technique: 


\begin{algorithm}[H]
    \caption{$\mathtt{FindUpper}(\epsilon)$}
    \label{alg:FindUpper}
    \begin{algorithmic}
        \STATE $t=1$
        \STATE $a_t=0$
        \STATE $a'_t=\epsilon$
        \WHILE{$\Psi(a_t, a_t) < \Psi(a'_t, a'_t)$}
            \STATE $t=t +1$
            \STATE $a_t=a'_{t-1}$
            \STATE $a'_t=a_t + 2^{t}\epsilon$
        \ENDWHILE
        \STATE Output $a'_t$.
    \end{algorithmic}
\end{algorithm}

\begin{theorem}
Then, $a'_t = \mathtt{FindUpper}(\epsilon)$ is such that $\alpha_A^*, \alpha_P^* \in [0, a'_t]$ and $t \le O(\log(\max(\alpha_A^*, \alpha_P^*)))$.
\end{theorem}
\begin{proof}
    \cj{TODO:}
\end{proof}

\subsection{Various Implementations for $\mathtt{DROJoinFixedAlphas}(\alpha_A, \alpha_P)$}

Current possible candidates are Proximal Gradient Descent, AMA, and ADMM. 


\cj{HERE}

For notational simplicity, we refer to problem \eqref{eqn:optimization1} with $\Omega(\alpha_A, \alpha_P, \theta)$:
\begin{align*}
    &\Omega(\alpha_A, \alpha_P, \theta)\\
    &= (\alpha_A r_A + \alpha_P r_P) + \frac{1}{n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \left(f(y^P_j\langle\theta, (x^A_i, a^A_i) \rangle) + \max(y^P_j\langle\theta, (\hat{x}_{i,j}, a^A_i) \rangle-\alpha_P\kappa_P,0) -\alpha_A||x^A_i -x^P_j|| \right) \\
    &+ \infty \ind[||\theta_1||_{*} \le \alpha_A + \alpha_P, ||\theta_2|_{*} \le \kappa_A \alpha_A, \alpha_A < \alpha_P].
\end{align*}
Also, we write $\Psi(\alpha_A, \alpha_P) = \min_{\theta}\Omega(\theta, \alpha_A, \alpha_P)$ and $\theta^*, \alpha^*_A, \alpha^*_P = \arg\min_{\theta, \alpha_A, \alpha_P} \Omega(\theta, \alpha_A, \alpha_P)$.



\cj{OLD STUFF BELOW: will recycle some stuff (e.g. AMA, ADMM)}
\subsection{Proximal(projected) Gradient Descent}
Our problem can be described as a convex optimization over intersection of convex sets: 
\begin{align*}
    \min_{\theta, \alpha_A, \alpha_P} f((\theta, \alpha_A, \alpha_P)) \\
    \text{s.t.} (\theta, \alpha_A, \alpha_P) \in C_1 \\
    (\theta, \alpha_A, \alpha_P) \in C_2,
\end{align*}
where in our case
\begin{align*}
    f(\theta, \alpha_A, \alpha_P) &= (\alpha_A r_A + \alpha_P r_P) + \frac{1}{n_A n_P} \sum_{i=1}^{n_A} \sum_{j=1}^{n_P} \left(f(y^P_j\langle\theta, (x^P_j, a^A_i) \rangle) + \max(y^P_j\langle\theta, (\hat{x}_{i,j}, a^A_i) \rangle-\alpha_P\kappa_P,0) -\alpha_A||x^A_i -x^P_j|| \right)\\
    C_1 &= \{(\theta, \alpha_A, \alpha_P): ||\theta_1||_{*} \le \alpha_A + \alpha_P, ||\theta_2|_{*} \le \kappa_A \alpha_A\}\\
    C_2 &= \{(\theta, \alpha_A, \alpha_P): \alpha_A < \alpha_P \}.
\end{align*}
